DRG: Dual Relation Graph for Human-Object Interaction Detection

We tackle the challenging problem of human-object interaction (HOI) detection. Existing methods either recognize the interaction of each human-object pair in isolation or perform joint inference based on complex appearance-based features. In this paper, we leverage an abstract spatial-semantic representation to describe each human-object pair and aggregate the contextual information of the scene via a dual relation graph (one human-centric and one object-centric). Our proposed dual relation graph effectively captures discriminative cues from the scene to resolve ambiguity from local predictions. Our model is conceptually simple and leads to favorable results compared to the state-of-the-art HOI detection algorithms on two large-scale benchmark datasets.

==> [ECCV 2020] HOI arXiv/0_abstract.tex <==
\begin{abstract}
%
% Problem
We tackle the challenging problem of human-object interaction (HOI) detection.
% Limitation
Existing methods either recognize the interaction of each human-object pair in isolation or perform joint inference based on complex appearance-based features.
In this paper, we leverage an abstract spatial-semantic representation to describe each human-object pair and aggregate the contextual information of the scene via a dual relation graph (one \emph{human-centric} and one \emph{object-centric}). 
Our proposed dual relation graph effectively captures discriminative cues from the scene to resolve ambiguity from local predictions.
% Outcomes
Our model is conceptually simple and leads to favorable results compared to the state-of-the-art HOI detection algorithms on two large-scale benchmark datasets.
\end{abstract}

%
% % What do we do? - context - Bipartite graph
% In this paper, we propose to use a bipartite graph to aggregate contextual information of the scene to resolve ambiguity from local predictions.
% %
% % What do we do? - spatial-semantic 
% We further leverage a spatial-semantic representation to describe each human-object pair.
% %
% We show that this simple abstract representation captures discriminative cues for recognizing HOI.

==> [ECCV 2020] HOI arXiv/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
% Problem
% - what's HOI
% - Why?
Detecting individual persons and objects in isolation often does not provide sufficient information for understanding complex human activities.
Moving beyond detecting/recognizing individual objects, we aim to detect persons, objects, and recognize their interaction relationships (if any) in the scene.
This task, known as human-object interaction (HOI) detection, can produce rich semantic information with visual grounding.

% Limitation
% - 1) App + Spatial (VSRL, HICO, InterACT, iCAN, Interactiveness, Alex's)
% - BUT, individual
% - 2) ECCV-GPNN, Graph RCNN, (some iterative passing)
% - BUT, complex feature, full graph
State-of-the-art HOI detection methods often use appearance features from the detected human/object instances as well as their relative spatial layout for predicting the interaction relationships~\cite{Chao-WACV-HOI,Gao-BMVC-iCAN,Gkioxari-CVPR-InteractNet,Gupta-SemanticRoleLabeling,Alex-No-Frills,Kolesnikov-BAR,Li-CVPR-Interactiveness, wang2019deep,zhou2019relation,Bo-PMFNet,peyre2018detecting,bansal2019detecting,liao2020ppdm}. 
These methods, however, often predict the interaction relationship between each human-object pair \emph{in isolation}, thereby ignoring the contextual information in the scene.
In light of this, several methods have been proposed to capture the contextual cues through iterative message passing~\cite{Qi-ECCV-GraphParsing,Xu-CVPR-MessagePassing} or attentional graph convolutional networks~\cite{Yang-ECCV-Graph-RCNN}.
However, existing approaches rely on complex appearance-based features to encode the human-object relation (e.g., deep features extracted from a union of two boxes) and do not exploit the informative spatial cues.
In addition, the contexts are aggregated via a \emph{densely connected} graph (where the nodes represent all the detected objects).
% Also, they construct the full graph of the scene to update appearances. This takes time and potentially involves unnecessary context.
% Our work
% - IN THIS WORK
% - our core idea,
%  1) S-S
%  2) Bipartite Graph: H and O subgraph
% - How good it is.

% \para{Our work.} 
%
In this paper, we first propose to use spatial-semantic representation to describe each human-object pair.
Specifically, our spatial-semantic representation encodes (1) the relative spatial layout between a person and an object and (2) the semantic word embedding of the object category.
Using spatial-semantic representation for HOI prediction has two main advantages:
First, it is invariant to complex appearance variations.
Second, it enables knowledge transfer among object classes and helps with rare interaction during training and inference.

% Context
While such representations are informative, predicting HOI in isolation fails to leverage the contextual cues.
In the example of \figref{teaser}, a model might struggle to recognize that the person (in the red box) is hitting the baseball, by using only the spatial-semantic features from this particular human-object pair.
Such ambiguity, however, may be alleviated if given the relation among different HOIs \emph{from the same person}, e.g., this person is wearing a baseball helmet and holding a baseball bat.
Similarly, we can exploit the relations among different HOIs \emph{from the same object}.
For example, a model may recognize both persons are holding the same baseball bat when making prediction independently.
Knowing that the person (red box) is more likely to hold the baseball bat reduces the probability of another person (blue box) holding the same baseball bat. 
Inspired by these observations, we construct a \emph{human-centric} and an \emph{object-centric} HOI subgraph and apply attentional graph convolution to encode and aggregate the contextual information.
We refer to our method as Dual Relation Graph (DRG).

% Hence, we construct an \emph{object-centric} HOI subgraph similar to the human-centric HOI subgraph.
%
% By combining both the \emph{human-centric} and \emph{object-centric} HOI subgraphs, we establish an effective graph-based method to aggregate HOI contextual information in the scene.
%
% We called our method Relation Bipartite Graph (RBG).

% While such representations are informative, predicting HOI in isolation inevitably suffers from ambiguity.
% %
% % We illustrate this limitation using an example on the right of \figref{teaser}.
% %
% Here, even though the spatial relationship between a person and a tennis racket looks similar, the presence of other objects in the scene and their spatial relationships with respect to the person provide discriminative signals for disambiguating the action the person is doing.
% % the type of action the person is performing \emph{without even considering the appearance of the person and objects}. 
% %
% For example, the spatial layout of the bench, the bag, and another person nearby suggests that the person may be resting instead of playing tennis.
% % 
% To capture the contextual cues, we present a \emph{human-centric} relation network to aggregate contextual information between a person and all objects in the scene.
% % 
% We refer to our model as Spatial-Semantic Aware Relation (SSAR) Network.
% %
% We validate the effectiveness of the proposed model using two large-scale HOI benchmarks and show favorable results against the state-of-the-art.
% 
% We also conduct a detailed ablation study to isolate the contributions from individual components.

% Contributions
\para{Our contributions.} 
\begin{compactitem}
\item We propose Dual Relation Graph, an effective method to capture and aggregate contextual cues for improving HOI predictions.

\item We demonstrate that using the proposed spatial-semantic representation alone (without using appearance features) can achieve competitive performance compared to the state-of-the-art.

\item We conduct extensive ablation study of our model, identifying contributions from individual components and exploring different model design choices.

\item We achieve competitive results compared with the state-of-the-art on the VCOCO and HICO-DET datasets.
\end{compactitem}




\ignorethis{
% OLD texts
% exploit the cues from such visual abstraction of the scene 
%
% \chen{How to make the following sentence more clear?}
% Specifically, we propose to use a spatial-semantic representation to encode the spatial relationship between a person and an object, as well as the semantic category embedding of the object he/she is interactive with.
%
% benefits of the semantic category embedding
% This abstract spatial-semantic representation is invariant to complex appearance variations.
% %
% Also, the use of semantic category embedding helps transfer knowledge among object classes. 
% %
% % For example, both elephant and horse are animals and can be ridden (with a similar spatial human-object layout).
% %
% Thus, the spatial-semantic representation of \emph{riding elephant} and \emph{riding horse} are close in the embedding space despite appearance differences. 
% 
% Better for zero-shot learning
This abstract representation will show its power on zero-shot learning. Furthermore, we believe naturally it is a perfect fit for the zero-shot task.


% \chen{I think we should replace object layout with interaction layout}
% What's the problem?
Recent years have witnessed rapid progress in visual recognition tasks, including object detection~\cite{Dai-NIPS-RFCN,Ross-CVPR-FastRCNN,Lin-CVPR-Pyramid,Ren-NIPS-FasterRCNN}, semantic and instance segmentation~\cite{Chen-TPAMI-DeepLab,Ross-CVPR-Hierarchies,He-ICCV-MaskRCNN,Long-CVPR-FCN}, and action recognition~\cite{Cheron-ICCV-PCNN,Girdhar-NIPS-AttentionalPooling,Maji-CVPR-Action}.
%
% Delete Gkioxari-ICCV-R*CNN Yao-CVPR-Combining because I want to emphasize these tasks focus on individual object.
These tasks, however, focus on characterizing \emph{individual} object instance, while neglecting the rich semantic information among these instances. 
%
Recently, the scene graph, a visually-grounded graphical structure of an image, is used to model the visual relationship among individual object instances~\cite{Hu-CVPR-Relation,Li-ICCV-SceneGraph,Newell-NIPS-Pixels,Xu-CVPR-MessagePassing,Yang-ECCV-Graph-RCNN,Yang-ECCV-Shuffle,Zellers-CVPR-Neural}, which leads to a deeper understanding of the scene.

% 
% HOI 
In this paper, we study a particularly important class of visual relationship detection, which detects how each person interacts with the surrounding objects. This task, known as Human-Object Interaction (HOI) detection~\cite{Chao-WACV-HOI,Gupta-SemanticRoleLabeling}, aims to localize a person, an object, as well as identify the interaction between the person and the object.
%
% Describe the input and output.
Given an image, we want to detect all the $\langle$ $\texttt{human, verb, object}$ $\rangle$ triplets.

% Why we should care about the problem?
Understanding Human-Object Interactions (HOIs) is an essential step towards a deeper understanding of the scene. Since most of the images are \emph{human-centric}, studying the HOI detection problem provides essential cues for high-level scene understanding tasks, such as pose estimation~\cite{Cao-CVPR-OpenPese,Yao-BMVC-Pose}, image captioning~\cite{Li-CVPR-Scene,Lu-CVPR-Baby}, and image retrieval~\cite{Johnson-CVPR-Retrieval}.

% Teaser
\input{figure/fig_teaser}

% Why existing approaches are not satisfactory?
With the rapid development of deep convolutional neural networks (DCNs), several methods~\cite{Chao-WACV-HOI,Gao-BMVC-iCAN,Gkioxari-CVPR-InteractNet,Gupta-SemanticRoleLabeling,Qi-ECCV-GraphParsing} have been proposed to tackle the problem.
%
These approaches, however, do not effectively encode the object layout information, which we argue is an informative cue for HOI detection.
%
Gkioxari~\etal~\cite{Gkioxari-CVPR-InteractNet} incorporates this geometric cue by regressing object location from human bounding box with a Mixture Density Network. Chao~\etal~\cite{Chao-WACV-HOI} encodes the relative location information using a two-channel binary image representation.
\yl{Not very sure about the claim.}
%
Both methods ignore the object category information when encoding the location information, which leads to a sub-optimal solution.
%
We argue that incorporating object category information could capture the location relation more effectively.
%
Thus, we explore a spatial-semantic feature representation by combining the spatial relation between a person and an object, and the object category information (encoded with pre-trained word embedding).
%


% 
In~\figref{teaser}, we show an example of detecting human-object interaction from the spatial layout between a person and an object, as well as the corresponding object categories. 
% %
% Inferring interactions from each H-O pair independently is commonly used in the HOI detection domain.
% \yl{Independently? Not really?}
% %
However, this local information is not discriminative enough and will cause ambiguities.
% %
Though the two persons highlighted in the white boxes share similar human-object spatial layout (\emph{center}), they are performing different actions (\emph{left}).
% %
% % What do we propose.
Thus, we leverage the \emph{global object layout} in the image (\emph{right}), which provides discriminative cues for inferring the interaction. Our intuition is that the global object layout serves as a complement to an individual HOI.
% %
% % Example shows why using the global object layout is good.
In the first example, the spatial layout between the person and the bench, the bag, and another person nearby together suggests that the person may be resting. 
% %
In the second example, the spatial layout of the person and tennis ball strongly indicator of hitting action.
% %
% Module overview 
In this paper, we propose the Spatial-Semantic Aware Relation (SSAR) module to aggregate features from a set of HOI instances, \eg all the interaction between the same person and other surrounding objects.
%
Inspired by~\cite{Hu-CVPR-Relation}, we adopt an attention mechanism to model the dependencies among HOIs. We measure the similarity between different HOIs in an end-to-end learnable embedding space and use it to get a weighted sum of the input features. 
%
Note that we can aggregate HOIs features iteratively by stacking more numbers of SSAR module.
%
We argue that using this non-appearance feature can achieve a reasonably good performance.


% A better S-S only baseline
% In this paper, we also explore a spatial-semantic feature representation by combining the spatial relation between a person and an object and the object category using pre-trained word embedding.
% \yl{This one should be in the last paragraph because this is how we construct the module?}
%
% We argue that using this non-appearance feature can achieve a reasonably good performance. The results are shown in the Table???
% % 
% In the spatial-semantic feature, we use the word embedded object category to capture the rich semantic relation between objects.
% %
% % Example of the advantage of S-S
% For example, the spatial relation of the action ``riding a horse" and ``riding an elephant" should look similar. And these two animals have closer distance in the word embedding space. 
% \yl{For the word embedding, is it really the case? How close are they?}

\paragraph{Our contributions.}
% Create a list of contributions. This helps the reviewers to summarize the paper. The rest of the paper provide evidences for the claimed novelty/contributions. Use forward references to provide a roadmap to the paper, e.g., we propose XXX (\secref{algorithm})

We make the following contributions.
\begin{itemize}
\item We propose the Spatial-Semantic Aware Relation (SSAR) module to refine interaction prediction iteratively 
\item We construct a strong baseline for HOI detection by using the spatial-semantic representation only.
\item With the full model, we establish new state-of-the-art performances on two HOI detection benchmarks
\item We conduct detailed ablation experiments to identify the relative contributions of each individual component.
\item We will release all the source code and pre-trained models to facilitate future research.
\end{itemize}
}

==> [ECCV 2020] HOI arXiv/2_related_work.tex <==
\section{Related Work}
\label{sec:related}
% === Tips === 
% - Use PRESENT tense to describe related work.
% - Avoid a laundry list of paper. A et al. propose X. B et al. propose Y. Instead, tell a story within each topic and cite relevant papers along the way.
% - Citations is NOT nouns. You cannot start a sentence with a citation (e.g. [1] proposes...). Your sentences should still make sense when you remove all the citations.
% - Do not just list related work. "Relate" them with this work. What's similar? What's different?
% - Example of citation: Huang~\etal~\cite{Huang-CVPR-2015}. The symbol "~" avoids breaking the words into different lines.

% === General structure within each topic ===
% (1) Introducing this topic. What's the input/output?

% (2) What other people have done in this topic?
% [Example] (Do not list! Organize!) 
% - Generative Adversarial Networks (GANs) [15, 62] have achieved impressive results in image generation [5, 37], image editing [65], and representation learning [37, 42, 35]. Recent methods adopt the same idea for conditional image generation applications, such as text2image [39], image inpainting [36], and future prediction [34], as well as to other domains like videos [53] and 3D data [56]. 

% (3) How our work RELATES to the papers in this topic? (Focus on "we", "our work", "our main focus")
% [Example] (for similar ideas)
% - Our work builds upon XXX and tackle the problem of XXX.
% - We use  XXX
% - In this work, we introduce a similar loss to XXX
% 
% [Example] (for different ideas)
% - In contrast to existing methods~\cite{XXX} that do XXX, we do XXX. We show that XXX ...
% - Existing approaches did XXX. Our main focus, on the other hand, is XXX
% - Unlike the above approaches, our formulation does not rely on XXX

% Motivation
\input{figure/fig_motivation}

\para{Human-object interaction detection.} 
The task of human-object interaction detection aims to localize persons, object instances, as well as recognize the interactions (if any) between each pair of a person and an object.
State-of-the-art HOI detection algorithms generally rely on two types of visual cues: 
(1) appearance features of the detected persons and objects (e.g., using the ROI pooling features extracted from a ConvNet) and 
(2) the spatial relationship between each human-object pair (e.g., using the bounding box transformation between the agent and the object~\cite{Gkioxari-CVPR-InteractNet,Gupta-SemanticRoleLabeling,Alex-No-Frills}, a two-channel interaction pattern~\cite{Chao-WACV-HOI,Gao-BMVC-iCAN}, or modeling the mutual contexts of human pose and object~\cite{Alex-No-Frills,Li-CVPR-Interactiveness,yao2010modeling}).
Recent advances focus on incorporating \emph{contexts} to resolve potential ambiguity in interaction prediction based on independent human-object pairs, including pairwise body-parts~\cite{Bo-PMFNet,fang2018pairwise} or object-parts~\cite{zhou2019relation}, instance-centric attention \cite{Gao-BMVC-iCAN,wang2019deep}, or message passing on a graph~\cite{Qi-ECCV-GraphParsing}.
Our work shares similar spirits with these recent efforts as we also aim to capture contextual cues.
The key difference lies in that the above approaches learn to aggregate contextual information from the other objects, body parts, or the scene background, while our method exploits  \emph{relations among different HOIs} to refine the predictions.

% Two stages
Inspired by the design of two-stage object detectors~\cite{Ren-NIPS-FasterRCNN}, recent works also show that filtering out candidate pairs with no relations using a relation proposal network~\cite{Yang-ECCV-Graph-RCNN} or an interactiveness network~\cite{Li-CVPR-Interactiveness} improves the performance.
Our method does not train an additional network for pruning unlikely relations.
We believe that incorporating such a strategy may lead to further improvement.

% Rare classes
Recent advances in HOI detection focus on tackling the long-tailed distributions of HOI classes. 
Examples include transferring knowledge from seen categories to unseen ones by an analogy transformation~\cite{Peyre-ICCV-Weakly}, performing data augmentation of semantically similar objects~\cite{bansal2019detecting}, or leveraging external knowledge graph~\cite{Kato_2018_ECCV}.
While we do not explicitly address rare HOI classes, our method shows a small performance gap between rare and non-rare classes. 
We attribute this to the use of our abstract spatial-semantic representation.

% The annotation distribution of HOIs is long-tailed, so we usually observe a performance drop between those rare classes and the common classes.
%
% To bridge this performance gap, Peyre~\etal~\cite{Peyre-ICCV-Weakly} proposes to transfer knowledge from seen categories to unseen ones by an analogy transformation.
% %
% Bansal~\etal~\cite{bansal2019detecting} exploit the fact that HOIs with semantic similar objects share a similar human-object spatial layout, to perform data augmentation during training explicitly.
%
% While we do not have special consideration for the rare categories in HOI, the performance gap between rare and non-rare classes is small.
% %
% Explicitly modeling the long-tailed behavior could potentially reduce the performance gap and improve the overall performance, which we will consider in our future work.

% \chen{Discuss shanghai JiaoTong's paper. But I don't know how to relate this paper to ours. Currently, we don't use two-stage architecture. But we can sort of take advantage of the interactiveness score.} Very recently, a two-stage method is proposed to detect HOIs~\cite{Li-CVPR-Interactiveness}. In the first stage, an interactiveness network is trained to predict the interactiveness between H-O pairs and suppress the less likely ones. The interactiveness prior can be learned across different HOI datasets. The second stage is a regular HOI detection model.

\para{Visual relationship detection.} 
Many recent efforts have been devoted to detecting visual relationships~\cite{Bilen-CVPR-Weakly,Dai-CVPR-Relationship,Hu-CVPR-Referential,Li-CVPR-VIP,Peyre-ICCV-Weakly,Zhang-ICCV-PPR,Zhuang-ICCV-ContextAware}.
Unlike object detection, the number of relationship classes can be prohibitively large due to the compositionality of object pairs, predicates, and limited data samples.
To overcome this issue, some forms of language prior have been applied~\cite{Lu-ECCV-Prior,Plummer-ICCV-Phrase}.
% How does HOI detection task differ from visual relationship detection task.
Our focus in this work is on one particular class of relationship: human-centric interactions.
Compared with other object classes, the possible interactions (the predicate) between a person and objects are significantly more fine-grained.
% 

\para{Scene graph.} 
A scene graph is a graphical structure representation of an image where objects are represented as nodes, and the relationships between objects are represented as edges~\cite{Newell-NIPS-Pixels,Xu-CVPR-MessagePassing,Yang-ECCV-Graph-RCNN,Yang-ECCV-Shuffle,Zellers-CVPR-Neural}. 
% Applications
As the scene graph captures richer information beyond categorizing scene types or localizing object instances, it has been successfully applied to image retrieval~\cite{Johnson-CVPR-Retrieval}, captioning~\cite{li2017scene}, and generation~\cite{johnson2018image}.
% Joint inferences
Recent advances in scene graph generation leverage the idea of iterative message passing to capture contextual cues and produce a holistic interpretation of the scene~\cite{Qi-ECCV-GraphParsing,Xu-CVPR-MessagePassing,Yang-ECCV-Graph-RCNN,Zellers-CVPR-Neural}. 
% Ours 
% Difference: 
%
% 1. each node is a HOI, not object
% 2. abstract feature, not appearance
% 3. human centric graph
%
Our work also exploits contextual information but has the following distinctions: 
%
(1) Unlike existing methods that apply message passing to update \emph{appearance features} (e.g., the appearance feature extracted from the union of human-object pair) at each step, we use an abstract spatial-semantic representation with an \emph{explicit} encoding of relative spatial layout.
%
(2) In contrast to prior works that use a single densely connected graph structure where edges connecting all possible object pairs,
% we adopt a \emph{human-centric} subgraph and an \emph{object-centric} subgraph.
we operate on human-centric and object-centric subgraphs to focus on relevant contextual information specifically for HOI. 
\figref{motivation} highlights the differences between methods that capture contextual cues. 
% which is faster and focus on a more relevant contextual information. 

The mechanisms for dynamically capturing contextual cues for resolving ambiguity in local predictions have also been successfully applied to sequence prediction~\cite{vaswani2017attention}, object detection~\cite{Hu-CVPR-Relation}, action recognition~\cite{girdhar2018video,Sun-CVPPR-Actor-centric,Wang-CVPR-2018}, and HOI detection~\cite{Gao-BMVC-iCAN}.
Our dual relation graph shares a similar high-level idea with these approaches but with a focus on exploiting the contexts of spatial-semantic representations.

% \chen{Not consistent.}
% HOIs of human-object pairs for a \emph{each specific person}.
% We propose to use a human-centric graph structure 
%
% We think a human should be the center of an action, and the nodes are connected only if the HOIs are performed by the same human.
% \jiabin{This does not explain anything. Why it SHOULD be this way? Simply describe what we did is not sufficient. Also, this is about describing DIFFERENCES. }

% % 1) We exploit the contextual information of the scene in the context of HOI. Each node is a HOI instead of an object.
% \jiabin{Please do not write incorrect statement! This is NOT an difference. All scene graph papers with joint inference have relationship as NODEs as well.}

% \paragraph{Capturing contexts.}
% The mechanisms that dynamically capture contextual cues for resolving ambiguity in local predictions have been successfully applied to object detection~\cite{Hu-CVPR-Relation}, action recognition~\cite{Wang-CVPPR-Non-local}, detection~\cite{girdhar2018video,Sun-CVPPR-Actor-centric}, and HOI detection~\cite{Gao-BMVC-iCAN}.

% Leveraging contextual information helps to relieve the ambiguity caused by predicting from local feature.
% %
% It has been successfully applied to object detection~\cite{Hu-CVPR-Relation}, action detection~\cite{girdhar2018video,Sun-CVPPR-Actor-centric,Wang-CVPPR-Non-local} and HOI detection\cite{Gao-BMVC-iCAN}.
%
% All these methods adopt an attention mechanism to attend over neighborhoods' features as the context for a more accurate detection.
% %
% Our work leverages contextual information in a human-centric manner.
% %
% HOIs performed by the same person can aggregate features from each other and yield a better prediction. \chen{It seems like this section can be combined with the previous section. I am not sure.}


% Recent advances focus on capturing contexts to resolve  potential  ambiguity  in interaction prediction based on independent human-object pairs,  including  pairwise  body-parts  [6],  instance-centric attention  [8],  or  message  passing  on  a  graph  [30].



% relation network for object detection~\cite{Hu-CVPR-Relation}
% graph attentional network~\cite{Bengio-Graph-attention}
% Non-local NN~\cite{Wang-CVPPR-Non-local}
% Video Action Transformer Network~\cite{girdhar2018video}
% iCAN~\cite{Gao-BMVC-iCAN}
% Actor-Centric Relation Network~\cite{Sun-CVPPR-Actor-centric}





% \chen{I also want to talk about relation network. Should I start a new section? I want to compare to relation network for object detection, non local NN, and graph convolutional network.}
% \jb{Sure, please start a new section.}


% Our work builds upon the scene graph model with an obvious distinction. We use a spatial-semantic feature to represent the interaction, in contrast to existing methods~\cite{Xu-CVPR-MessagePassing} that use the union appearance feature to represent the interaction. We argue the spatial information is informative.
% 
% We explore the relation between different interaction directly, in contrast to the relation network~\cite{Hu-CVPR-Relation} which leverages the relation between different objects.


% Scene graph has attracted much attention due to its ability to capture complex information and their applicability to 
% 
% Recently scene graph have shown its power in object detection~\cite{Hu-CVPR-Relation} and relation detection ~\cite{Xu-CVPR-MessagePassing,Yang-ECCV-Graph-RCNN,Newell-NIPS-Pixels,Yang-ECCV-Shuffle,Zellers-CVPR-Neural}.
%
% It is shown that incorporating the rich relationships between objects helps with object detection\cite{Hu-CVPR-Relation}. 
% % 
% Later, Xu~\etal~\cite{Xu-CVPR-MessagePassing} proposed a model which consists of two subgraphs that alternately perform message passing for object and relations. These two subgraphs jointly infer and make predictions on objects and their relationships. 
% %
% Inspired by this joint graph inference, more works are conducted to benefit from jointly solving vision tasks. Li~\etal~\cite{Li-ICCV-SceneGraph} proposed a multi-level scene description network that jointly solve an object detection, a scene graph generation and a region captioning task. In their work, mutual connections across different semantic levels are considered. Messages are passed across the three levels of semantic tasks through the graph.
% %
% Recently, scene graph has been borrowed to solve HOI detection problem. Graph-propagation methods were used for message passing and thus leads to a better feature representation~\cite{Yang-ECCV-Graph-RCNN,Qi-ECCV-GraphParsing}.
% %
% The interaction is represented by the union feature of human and object. And the information is passing between objects and interactions through edges and integrates other nodes' information. In order to automatically prune the unlikely edges in the graph, Yang~\etal~\cite{Yang-ECCV-Graph-RCNN} includes a proposal sub-network which prunes unlikely relationship edges, making the whole network end-to-end trainable.

% % Ours
% Our work builds upon the scene graph model with an obvious distinction. We use a spatial-semantic feature to represent the interaction, in contrast to existing methods~\cite{Xu-CVPR-MessagePassing} that use the union appearance feature to represent the interaction. We argue the spatial information is informative.
% % 
% We explore the relation between different interaction directly, in contrast to the relation network~\cite{Hu-CVPR-Relation} which leverages the relation between different objects.

% Don't know how to relate these two works.
%
% Zellers~\etal~\cite{Zellers-CVPR-Neural} proposed a scene graph that leverages regularly appearing substructures. Also, this paper proposed a statistics baseline: given object detections, predict the most frequent relation between object pairs with the given labels.
% 
% Newell~\etal~\cite{Newell-NIPS-Pixels} proposed a special graph called full graph where each pixel in an image is a node. This full graph overcomes the isolation of each  individual pair of objects.

% Limitation
% All of the aforementioned methods have a common drawback. There is no direct communication between different relationships. For example, knowing a person is wearing a baseball cap will be helpful for detecting this person holding a baseball bat.

\para{Visual abstraction.} 
The use of visual abstraction helps direct the focus to study the semantics of an image~\cite{zitnick2013bringing}.
Visual abstraction has also been applied to learn common sense~\cite{vedantam2015learning}, forecasting object dynamics~\cite{fouhey2014predicting}, and visual question answering~\cite{yi2018neural}. 
Our work leverages the contexts of an abstract representation between human-object pairs for detecting HOIs.

\para{Spatial-semantic representation.} 
% Spatial or spatial-semantic representation have been exploited in the context of human-object interactions. 
% The spatial relationship between a person and an object can be either encoded by a normalized two-channel interaction pattern~\cite{Chao-CVPR-HICO,Gao-BMVC-iCAN}, 4D bounding box transformation~\cite{Gkioxari-CVPR-InteractNet,Gupta-SemanticRoleLabeling}, or the mutual context of human pose and object location~\cite{yao2010modeling,Alex-No-Frills}. 
Spatial-semantic representation has also been applied in other problem domains such as image search~\cite{mai2017spatial}, multi-class object detection~\cite{desai2011discriminative}, and image captioning~\cite{yin2017obj2text}.

%% Detail summaries
% \\
% ---------------------------------------------
% \\
% Deep Contextual Attention for Human-Object Interaction Detection \cite{wang2019deep}
% [contextual attention]

% 1 generate contextual appearance feature to capture larger filed of view information by larger convolutional kernel (LK)
% 2 then apply contextual attention to contextual appearance feature in order to mitigate noise of background [dot product]
% 3 use a attention refinement block to further apply spatial and channel-wise attention
% \\
% ----------------------------------------------------
% \\
% - Relation parsing neural network for human-object interaction detection \cite{zhou2019relation}
% [Body part graph attention]

% 1 use two attention graphs: Object-Body part graph and human-body part graph
% 2 Object-Body part graph is used for aggregating information of human body parts and objects 
% 3 Human-body part graph assumbles information from human body parts and human
% 4 difference with our work: 
% They are leveraging correlations between human body parts and objects.
% We build graphs for each human object pair and leverage relationships between different pairs.
% \\
% -----------------------------------------------
% \\
% - Pose-aware Multi-level Feature Network for Human Object Interaction Detection \cite{Bo-PMFNet}
% [pose keypoint attention]

% Main Contribution
%     1 Use a Zoom-in Module to capture local human features at human pose keypoints
%     2 Add coordinate map to align & Use an attention network to weight each keypoint local features
% Intuition
%     1 Interactions have strong correlations with spatial location of human parts and object, e.g. if "hand" close to object, interaction is likely to be "hold" or "carry"
% Method
%     1 Holistic Module: capture coarse features and predict interactiveness
%     2 Zoom-in Module: capture fine features. Combine with Holistic Module to predict actions.
% \\
% -----------------------------------------------
% \\
% - Detecting unseen visual relations using analogies\cite{peyre2018detecting}

% 1 aim at detecting unseen relations by transferring knowledge from seen triplets to unseen triplets.

% 2 propose to learn representation of visual relations from visual embedding and phrase embedding. 

% 3 At training time, the network learns to map paired visual features and language representation to the same latent space.

% 4 At test time, the embedding of an unseen triplet is estimated from an analogy transformation trained by seen triplets. 
% Then the embedding is used to retrieve related images by finding the nearest neighbor in visual representation space.
% \\
% -----------------------------------------------
% \\
% - Detecting Human-Object Interactions via Functional Generalization \cite{bansal2019detecting}
% 1 measure function similarities between objects
% 2 use word embedding

% ---------------------------------------------


% ===================================
% Opening. 
% \ignorethis{
% Detecting HOI provides a deeper understanding of the activity in a scene.
% % Talk about the original Semantic role labeling paper.
% Gupta and Malik~\cite{Gupta-SemanticRoleLabeling} first tackle the HOI detection problem --- detecting people doing actions and the object instances they are interacting with.
% %
% Associating objects in a scene to various semantic roles with the action leads to a finer-grained understanding of the current state of activity.
% \yl{Why do we need this sentence here?}
% % Talk about InteractNet
% Gkioxari~\etal~\cite{Gkioxari-CVPR-InteractNet} extend the method in \cite{Gupta-SemanticRoleLabeling} by introducing action-specific density over target object locations based on the appearance of a detected person. 
% % 
% Significantly improved results have also been shown by replacing feature backbone with ResNet-50~\cite{He-CVPR-ResNet} and the Feature Pyramid Network~\cite{Lin-CVPR-Pyramid}.
% % Talk about HO-RCNN
% In addition to using object instance appearance, Chao~\etal~\cite{Chao-WACV-HOI} also encode the relative spatial relation between a person and the object with a two-layer CNN.
% %
% % Talk about iCAN
% Very recently, Gao~\etal~\cite{Gao-BMVC-iCAN} proposed an instance-centric attention module which extracts contextual features complementary to appearance features of the localized regions to facilitate HOI detection.
% }



==> [ECCV 2020] HOI arXiv/3_method.tex <==
\section{Method}
\label{sec:overview}
% \jiabin{Need some high-level motivation description for the dual graph.}
\input{figure/fig_overview}

% Overview of the network
In this section, we present our network for HOI detection (\figref{overview}).
We start with an overview of our network (\secref{alg_overview}). 
We then introduce the spatial-semantic representation (\secref{s-s_feature}) and describe how we can leverage the proposed Dual Relation Graph (DRG) to propagate contextual information (\secref{RBG}). 
% Next, we describe the Spatial-Semantic Aware module (\secref{SSAM}). 
Finally, we outline our inference (\secref{inference}) and the training procedure (\secref{training}).

\subsection{Algorithm overview}
\label{sec:alg_overview}

% Object detection  As illustrated in Figure 1, 
\figref{overview} provides a high-level overview of our HOI detection network.
%
We decompose the HOI detection problem into two steps: (1) object detection and (2) HOI prediction.
Following Gao \etal~\cite{Gao-BMVC-iCAN}, we first apply an off-the-shelf object detector Faster R-CNN~\cite{Ren-NIPS-FasterRCNN} to detect all the human/object instances in an image.
We denote $\mathbb{H}$ as the set of human detections, and $\mathbb{O}$ as the set of object detections. 
Note that ``person'' is also an object category.
We denote $b_h$ as the detected bounding box for a person and $b_o$ for an object instance.
We use $s_h$ and $s_o$ to denote the confidence scores produced by the object detector for a detected person $b_h$ and an object $b_o$, respectively. 
Given the detected bounding boxes $b_h$ and $b_o$, we first extract the ROI pooled features and pass them into the human and object stream.
We then pass the detected bounding boxes as well as the object category information to the spatial-semantic stream. 
We apply the proposed \emph{Dual Relation Graph (DRG)} in the spatial-semantic stream.
Lastly, we fuse the action scores from the three streams (human, object, and spatial-semantic) to produce our final predictions.

\para{Human and object stream.} 
% 
% Input is appearance feature
%Both human and object stream takes appearance feature and predicts the HOI independently.
Our human/object streams follow the standard object detection pipeline for feature extraction and classification.
For each ROI pooled human/object feature, we pass it into a 
one-layer MLP followed by global average pooling and obtain the human appearance feature $\bold{f}_h$ and the object appearance feature $\bold{f}_o$.
We then apply a standard classification layer to obtain the A-dim action scores $s_h^a$ (from human stream) and $s_o^a$ (from object stream).

\para{Spatial-semantic stream.} 
Our inputs to this stream are the spatial-semantic features (described in \secref{s-s_feature}).
In an image, we pair all the detected persons in $\mathbb{H}$ with all the objects in $\mathbb{O}$, and extract spatial-semantic features for each human-object pair.
We then pass all the features into our proposed Dual Relation Graph (\secref{RBG}) to aggregate the contextual information and produce updated features for each human-object pair.
Our dual relation graph consists of a human-centric subgraph and an object-centric subgraph.
These two subgraphs produce the action scores, $s_{spH}^a$ and $s_{spO}^a$.


\input{figure/fig_bipartite}
\vspace{-4.0mm}
\subsection{Spatial-semantic representation}
\label{sec:s-s_feature}

We leverage the \emph{abstract visual representation} of human-object pair for HOI prediction.
The visual abstraction of a human-object pair allows us to construct representations that are invariant to intra-class appearance variations.
In the context of human-object interaction, we consider the two important visual abstractions: (1) spatial relationship and (2) object category.
\footnote{Other types of abstracted representation such as the pose of the person, the attribute of the person/object can also be incorporated into our formulation. We leave this to future work.}  

\para{Capturing pairwise spatial relationship.} 
Following \cite{Chao-WACV-HOI,Gao-BMVC-iCAN}, we use the two-channel binary image representation to model the spatial relationship between a person and an object.
To do so, we take the union of the two bounding boxes as a reference and rescale it to a fixed size.
A binary image with two channels can then be created by filling value ones within the human bounding box in the first channel and filling value ones within the object bounding box in the second channel.
The remaining locations are then filled with value 0.
We then feed these two-channel binary images into a simple two-layer ConvNet to extract the spatial relation feature.

\para{Capturing object semantics.} 
We find that using spatial features by itself leads to poor results in predicting the interaction. 
To address this issue, we augment the spatial feature with the word embedding of each object's category, $vector$($o$), using fastText~\cite{Mikolov-LREC-fastText}.
Let $\bold{x}_{ij}$ denote the \emph{spatial-semantic feature} between the $i$-th person and the $j$-th object. We construct $\bold{x}_{ij} \in \mathbb{R}^{5708}$ by concatenating (1) the spatial feature and (2) the $ 300$-dimensional word embedding vector.

\subsection{Dual Relation Graph}
\label{sec:RBG}
%
Here, we introduce the Dual Relation Graph for aggregating the spatial-semantic features.
%
\figref{bipartite_graph} illustrates the overall process.

\heading{Relation graph.}
Given the object detection results, \ie instances in $\mathbb{H}$ and $\mathbb{O}$, we construct a relation graph (\figref{bipartite_graph}b). 
There are two types of nodes in this graph, $\mathbb{H}$ (human) and $\mathbb{O}$ (object). 
For each node $\textit{h}$ in $\mathbb{H}$, we connect it to all the other nodes in $\mathbb{O}$. 
Similarly, for each node $\textit{o}$ in $\mathbb{O}$, we connect it to all nodes in $\mathbb{H}$.

\heading{Human-centric subgraph and object-centric subgraph.}
Unlike previous methods \cite{Qi-ECCV-GraphParsing, Yang-ECCV-Graph-RCNN}, we do not use the densely connected graphs.
To exploit the relation among different HOIs performed by \emph{the same person}, we construct a \emph{human-centric} subgraph. 
Similarly, we construct an \emph{object-centric} subgraph for the HOIs performed on \emph{the same object} (\figref{bipartite_graph}c).
So far, each node stands for an object instance detection. 
To explicitly represent the HOI, we insert an HOI node $\it{x_{ij}}$ between each paired human node $\it{h_i}$ and object node $\it{o_j}$. 
We then connect all the HOI nodes and obtain \emph{human-centric} HOI subgraph and \emph{object-centric} HOI subgraph (\figref{bipartite_graph}d). 
We use the before mentioned \emph{spatial-semantic feature} $\bold{x}_{ij}$ to encode each HOI node between the $i$-th person and the $j$-th object.
% The representation of each HOI node is the before mentioned \emph{spatial-semantic feature} between the $i$-th person and the $j$-th object, $\bold{x}_{ij}$.

% \input{figure/fig_bipartite}

\heading{Contextual feature aggregation.}
% 
With these two HOI subgraphs, we follow a similar procedure for propagating and aggregating features as in relation network~\cite{Hu-CVPR-Relation}, non-local neural network~\cite{Wang-CVPR-2018}, and attentional graph convolutional network~\cite{Yang-ECCV-Graph-RCNN}.
%

\emph{Human-centric HOI subgraph}. To update node $\it{x_{ij}}$, we aggregate all the spatial-semantic feature of the nodes involving the same $i$-th person $\{x_{ij^\prime}| j^\prime \in \mathcal{N}(j)\}$. 
% 
%  node: \textit{ho} \textit{$h_i o_j$}
%  feature: $\bold{h}_{i}\bold{o}_{j}$
% subgraph and perform iterative message passing via graph convolution operators. \chen{Need to finalize the term. human-centric HOI subgraph; human subgraph}
% 
% \chen{Change $\bold{h}_{i}\bold{o}_{j}$ to $x_{ij}$.} 
The feature aggregation can be written as:
% 
\begin{equation} \label{eq:feature_updating}
\bold{x}_{ij}^{(l+1)} = \sigma \left( \bold{x}_{ij}^{(l)} + \sum_{j^\prime \in \mathcal{N}(j)} \alpha_{j j^\prime} W \bold{x}_{ij^\prime}^{(l)}\right), 
\end{equation}
where $W \in \mathbb{R}^{5708 \times 5708}$ is a learned linear transformation that projects features into the embedding space, $\alpha_{i j^\prime}$ is a learned attention weight. 

We can rewrite this equation compactly with matrix operation: 
% \chen{vectorize alpha, u}
% 
\begin{align} \label{eq:feature_updating_matrix}
\bold{x}_{ij}^{(l+1)} & = \sigma \left( W X^{(l)} \bm{\alpha}_j\right) \\
u_{jj^\prime} & = \left(W_q \bold{x}_{ij^\prime}^{(l)}\right)^\top \left(W_k \bold{x}_{ij}^{(l)} \right) / \sqrt{d_k} \\
\bm{\alpha}_j & = \text{softmax} (\bm{u}_{j}),
\end{align}
% Introduce Query, Key, Value, 
where $W_q, W_k \in \mathbb{R}^{1024 \times 5708}$ are linear projections that project feature into a query and a key embedding space. 
Following~\cite{vaswani2017attention}, we calculate the attention weights using scaled dot-product, normalized by $\sqrt{d_k}$ where $d_k = 1024$ is the dimension of the key embedding space.
We do not directly use the aggregated feature $\sigma \left( W X^{(l)} \bm{\alpha}_j\right)$ as our output updated feature. Instead, we add it back to the original spatial-semantic feature $\bold{x}_{ij}^{(l)}$.
We then pass the addition through a LayerNorm to get the final aggregated feature on the human-centric subgraph.
\begin{equation} \label{eq:updating}
\bold{x}_{ij}^{(l+1)} = \text{LayerNorm}\left(\bold{x}_{ij}^{(l)} + \sigma \left( W X^{(l)} \bm{\alpha}_j\right) \right).
\end{equation}
%

The linear transformation $W$ does not change the dimension of the input feature, thus the output $\bold{x}_{ij}^{(l+1)}$ has the same size as input $\bold{x}_{ij}^{(l)}$.
As a result, we can perform several iterations of feature aggregation (\figref{bipartite_graph}e). 
We explore the effectiveness of more iteration in \tabref{ablation}(a).\\

\emph{Object-centric HOI subgraph}. Similarly, to update node $\it{x_{ij}}$, we aggregate all the spatial-semantic feature of the nodes which involved the same object $\{x_{i^\prime j}| i^\prime \in \mathcal{N}(i)\}$. 
The two subgraphs have independent weights and aggregate contextual information independently.


\subsection{Inference}
\label{sec:inference}
%
% Given an input image, our model predicts HOI scores in a similar manner to the existing methods~\cite{Gao-BMVC-iCAN,Gkioxari-CVPR-InteractNet,Gupta-SemanticRoleLabeling}.
%
For each human-object bounding box pair ($b_h$, $b_o$) in image $I$, we predict the score $S^a_{h,o}$ for each action $a \in \left\{ 1, \cdots, A \right\}$, where $A$ denotes the total number of possible actions.
The final score $S^a_{h,o}$ depends on  
(1) the confidence for the individual object detections ($s_h$ and $s_o$), 
(2) the prediction score from the appearance of the person $s^a_h$ and the object $s^a_o$, and 
(3) the prediction score based on the aggregated spatial-semantic feature, using human-centric and object-centric subgraph, $s_{spH}^a$ and $s_{spO}^a$.
We compute the HOI score $S^a_{h,o}$ for the human-object pair ($b_h$, $b_o$) as
%
\begin{align}    
S^a_{h,o} & = s_h \cdot s_o \cdot s^a_{h} \cdot s^a_{o} \cdot s^a_{spH} \cdot s^a_{spO}
\end{align}
%
Note that we are not able to obtain the action scores using object $s^a_{o}$ or the spatial-semantic stream for some classes of actions as they do not involve any objects (\eg walk, smile).
For those cases, we use only the score $s^a_h$ from the human stream.
For those actions, our final scores are $s_h \cdot s^a_h$.

\subsection{Training}
\label{sec:training}
%
HOI detection is a multi-label classification problem because a person can simultaneously perform different actions on different objects, e.g., sitting on a chair and reading a book.
Thus, we minimize the cross-entropy loss \emph{for each individual action class} between the ground-truth action label and the score produced from each stream. 
The total loss is the summation of the loss at each stream.

==> [ECCV 2020] HOI arXiv/4_result.tex <==
\section{Experimental Results}
\label{sec:results}
\input{figure/fig_visual}
In this section, we first outline our experimental setup, including datasets, metrics, and implementation details. 
We then report the quantitative results on two large-scale HOI benchmark datasets and compare the performance with the state-of-the-art HOI detection algorithms.
Next, we show sample visual results on HOI detection. 
We conduct a detailed ablation study to quantify the contributions from individual components and validate our design choices.
More results can be found in the supplementary material.
We will make the source code and pre-trained models publicly available to foster future research.

\input{table/VCOCO_results}

\subsection{Experimental setup}
\para{Datasets.}
% Describe datasets used, statistics (# images, train/test splits)
%
\tb{V-COCO dataset}~\cite{Gupta-SemanticRoleLabeling} is constructed by augmenting the COCO dataset~\cite{Lin-ECCV-MSCOCO} with additional human-object interaction annotations.
%
% V-COCO consists of a total of 10,346 images containing 16,199 human instances. 
%
Each person is annotated with a binary label vector for 29 different action categories (five of them do not involve associated objects).
%
\tb{HICO-DET}~\cite{Chao-CVPR-HICO} is a larger dataset containing 600 HOI categories over 80 object categories (same as \cite{Lin-ECCV-MSCOCO}) with more than 150K annotated instances of human-object pairs.
%
% Note: we arrange the dataset a little bit.
For applying our method on the HICO-DET dataset, we disentangle the 600 HOI categories into 117 object-agnostic action categories and train our network over these 117 action categories.
At test time, we then combine the predicted action and the detected object and convert them back to the original 600 HOI classes.
Note that the evaluation for the HICO-DET dataset remains the same.
%
% As there is no official \emph{validation} set, we randomly sample $10\%$ of the training data as the \emph{val} set.

\para{Evaluation metrics.}
% Describe how you evaluate the performance
To evaluate the performance of our model, we adopt the commonly used role mean average precision (role mAP)~\cite{Gupta-SemanticRoleLabeling} for both V-COCO and HICO datasets.
% We evaluate the HOI detection performance using the commonly used role mean average precision (role mAP)~~\cite{Gupta-SemanticRoleLabeling} for both V-COCO and HICO datasets.
%
The goal is to detect and correctly predict the $\langle$ $\texttt{human, verb, object}$ $\rangle$ triplet.
% The goal is to detect the agent and the objects in the various roles for the action, denoted as the $\langle$ $\texttt{human, verb, object}$ $\rangle$ triplet. 
%
We consider a triplet as true positive if and only if it localizes the human and object accurately (\ie with IoUs $\geq 0.5$ w.r.t the ground truth annotations) and predicts the action correctly.
% A detected triplet is considered as a true positive if it has the correct action label, and both the predicted human and object bounding boxes $b_h$ and $b_o$ have IoUs $\geq 0.5$ w.r.t the ground truth annotations.

\input{table/HICO_results}
% \input{table/HICO_zeroshot}
% \input{figure/fig_multi_action}

\para{Implementation details.} 
%
% We build our network upon the publicly available official implementation of iCAN~\cite{Gao-BMVC-iCAN}.\footnote{\url{https://github.com/vt-vl-lab/iCAN}}
We build our network with the publicly available PyTorch framework.
Following Gao~\etal~\cite{Gao-BMVC-iCAN}, we use the Detectron \cite{Detectron} with a feature backbone of ResNet-50 to generate human and object bounding boxes.
For VCOCO, we conduct an ablation study on the validation split to determine the best threshold. We keep the detected human boxes with scores $s_h$ higher than 0.8 and object boxes with scores $s_o$ higher than 0.1. 
For HICO-DET, since there is no validation split available, we follow the setting in \cite{peyre2018detecting}. We use the score threshold 0.6 to filter out unreliable human boxes and threshold 0.4 to filter out unconfident object boxes.
To augment the training data, we apply random spatial jitterring to the human and object bounding boxes and ensure that the IOU with the ground truth bounding box is greater than 0.7.
We pair all the detected human and objects, and regard those who are not ground truth as negative training examples. 
We keep the negative to positive ratio to three.

% Network training detail
% We initialize our appearance feature backbone with the COCO pre-trained weight from Faster R-CNN \cite{Ren-NIPS-FasterRCNN}.
We initialize our appearance feature backbone with the COCO pre-trained weight from Mask R-CNN \cite{He-ICCV-MaskRCNN}.
We perform two iterations of feature aggregation on both \emph{human-centric} and \emph{object-centric} subgraphs. 
We train the three streams (human appearance, object appearance, and spatial-semantic) using the V-COCO \emph{train} set.
We use early stopping criteria by monitoring the validation loss.
% The first two streams of our network, namely human stream and object stream, are trained together, while the spatial-semantic stream is trained alone. 
% for 540K iterations 
We train our network with a learning rate of $0.0025$, a weight decay of $0.0001$, and a momentum of $0.9$ on both the V-COCO \emph{train} set and HICO-DET \emph{train} set. 
Training our network takes $14$ hours on a single NVIDIA P100 GPU on V-COCO and $24$ hours on HICO-DET.
% 
% HICO-DET
% for 820K iterations
% We train our network on the HICO-DET \emph{train} set with a learning rate of $0.01$, a weight decay of $0.0001$, and a momentum of $0.9$.
% Training our model on HICO-DET takes $24$ hours.
%
At test time, our model runs at $3.3$ fps for VCOCO and $5$ fps for HICO-DET.
% \yl{Jiarui, please update the training time.}

% \jiabin{Report runtime at the TEST time here.}

\subsection{Quantitative evaluation}
% Comparison to the state-of-the-art

% \input{table/VCOCO_results}
% \input{table/HICO_results}
We report the main quantitative results in terms of $AP_{role}$ on V-COCO in \tabref{vcoco_comparison} and HICO-DET in \tabref{HICO}.
For the V-COCO dataset, our method compares favorably against state-of-the-art algorithms~\cite{Li-CVPR-Interactiveness,wang2019deep,zhou2019relation} except PMFNet \cite{Bo-PMFNet}, which uses human pose as an additional feature.
Since pose estimation required additional training data (with pose annotations), we expect to see performance gain using human pose.
PMFNet \cite{Bo-PMFNet} also reports the $AP_{role}$ \emph{without} human pose, which is $2.4$ mAP lower to our method. 
% 
We also note that the spatial-semantic stream alone \emph{without} using any visual features achieves a competitive performance ($47.1$ mAP) when compared with the state-of-the-art. 
This highlights the effectiveness of the abstract spatial-semantic representation and contextual information.
Compared with methods that perform joint inference on densely connected graph~\cite{Qi-ECCV-GraphParsing},
% \jiabin{Cite }
our approach produces significant performance gains.

% HICI-DET qualitative evaluation
For the HICO-DET dataset, our method also achieves competitive performance with state-of-the-art methods~\cite{Alex-No-Frills,Li-CVPR-Interactiveness,Bo-PMFNet,Peyre-ICCV-Weakly}.
Our method achieves the best performance for the \emph{rare categories}, showing that our method handles the long-tailed distributions of HOI classes well.
% , highlighting the effectiveness of the proposed abstract spatial-semantic feature. 
% \chen{Rewrite this section once the s-s only result is updated.}

% We report our results with ResNet-50 and ResNet-152 backbones for a fair comparison with existing methods. 
We note that the current best performing model~\cite{bansal2019detecting} uses an object detector which is fine-tuned on HICO-DET \emph{train} set using the annotated object bounding boxes.
For a fair comparison, we also fine-tune our object detector on HICO-DET and report our result.
Note that we do \emph{not} re-train our model, but only replace the object detector at the test time.

Here, the large performance gain from fine-tuning the object detector may not reflect the progress on the HOI detection task.
This is because the objects (and the associated HOIs) in the HICO-DET dataset are \emph{not} fully annotated. 
Using a fine-tuned object detector can thus improve the HOI detection performance by exploiting such annotation biases. 
% As the objects in the HICO-DET dataset is not fully annotated, 
% \yl{Revisit here later when we have the final numbers.}

% \subsection{Zero-shot setting evaluation}
% We also evaluate our method on HICO-DET under the zero-shot setting to validate the effectiveness of using a semantic word embedding for transferring knowledge among object classes.
% %
% % The use of the semantic word embedding helps transfer knowledge among object classes.
% %
% For example, we may only see training examples where a person is riding an elephant but not a horse.
% %
% However, both elephant and horse are animals and can be ridden (with a similar spatial human-object layout).
% %
% Thus, the spatial-semantic representation of \emph{riding elephant} and \emph{riding horse} are close in the embedding space despite large appearance differences.
% %
% At testing, our model may still predict the \emph{riding} action for \emph{riding horse} even though no examples of a person riding a horse are available during training.
% % a reasonable \emph{riding} score for \emph{riding horse}, even though we never see this training example before.

% % How I prepapre the training data

% \para{Experimental setup}
% Following \cite{Shen-WACV-Zeroshot}, we omit 120 HOI categories and only train our network with the remaining 480 HOI categories.
% %
% We randomly choose the 120 categories and ensure that every verb or object within the 120 categories shows up at least once in the 480 HOI categories.
% % During training, we omit 120 HOI categories and only train our network with a subset of HICO-DET training images which contains the remaining 480 HOI categories. 
% % To evaluate, we calcualte the mAP of the omitted 120 HOI categories on the testing set.
% % %
% % Similar to~\cite{Shen-WACV-Zeroshot}, we do not cherry pick these 120 categories. We randomly choose 120 categories and only ensure that every verb or object within the 120 categories shows up at least once in the training categories.

% We report the quantitative results in terms of mAP on HICO-DET in \tabref{HICO_zero_shot}.
% % 1. fastText is better than one-hot vector
% % 2. S-S is better than App.
% % 3. S-S is complementary to App.
% Our proposed spatial-semantic feature with fastText word embedding~\cite{Mikolov-LREC-fastText} leads to an absolute gain of $1.73$ mAP compared to using one-hot vector.
% %
% When combined with human appearance stream, our model leads to a sizable performance boost, showing that our spatial-semantic feature is complementary to appearance features. 
% % It is also worth noting that only using spatial-semantic feature performs better than using human appearance feature.
% %
% % Thus, our spatial-semantic feature is a good complementary to the appearance feature.
% % \jb{This is not a logical statement. A is better than B. How did you reach the conclusion that A is complementary with B?}
\vspace{-2.0mm}
\subsection{Qualitative evaluation}

% \input{figure/fig_visual}
% \input{figure/fig_multi_action}

% Show visual results
\para{HOI detection results.}
Here we show sample results on the V-COCO dataset and the HICO-DET dataset in \figref{visual}. % (in \figref{HICO}).
%
We highlight the detected person and the associated object with red and green bounding boxes, respectively.
%
% \figref{multi_action} shows examples of detecting persons simultaneously performing multiple actions and associating the detected object instances to their semantic roles of the action. 
% \yl{Might remove this figure?}

\input{figure/fig_RBG}
\input{table/VCOCO_ablation}
\para{Visualizing the effect of the Dual Relation Graph.} 
In \figref{RBG}, we show the effectiveness of the proposed DRG. 
In the first two rows, we show that by aggregating contextual information, using the  \emph{human-centric} subgraph produces more accurate HOI predictions.
% For example, the human in the top left image is cutting a cake. 
% Without \emph{human-centric} feature aggregation, the model predicts a low score for the action "cut". By iteratively aggregating the information from other human-object pairs of this human, our model learns to infer the action more and more accurately.
%
Another example in the top right image indicates that the \emph{human-centric} subgraph can also suppress the scores for unrelated human-object pairs. 
% The example shows that our model can predict a low score for the girl lying in the table, and our model is able to generate lower scores with more iterations.
%
In the bottom two rows, we show four examples of how the \emph{object-centric} subgraph propagates contextual information in each step to produce increasingly more accurate HOI predictions.
%
For instance, the bottom right images show that for a person and an object without interaction, our model learns to suppress the predicted score by learning from the relationship of other HOI pairs associated with this particular object (laptop). 
In this example, the model starts with predicting a high score for the woman working on a computer. 
By learning from the relationship between the man and the computer, our model suppresses the score in each iteration.
% \chen{Explain with the real example.}


% \paragraph{Sample detection results.}

% \figref{relation} shows some representative examples with high relation weights. 
% 
% The first example shows that knowing the interaction with the surrounding objects helps with making a plausible prediction, \eg, the person is not hitting with a tennis racket.
% \yl{waiting for all the figures. Do we need Fig6 if we already have Fig8?}

% \input{figure/fig_Relation_Compare}
\subsection{Ablation study}
\label{sec:ablation}
We examine several design choices using the V-COCO \emph{val} set.

% Evaluate the individual contribution of each component
\para{More iteration of feature aggregation.} 
\tabref{ablation}(a) shows the performance using different iterations of feature aggregation.
For either \emph{human-centric} or \emph{object-centric} subgraph, using more iterations of feature aggregation improves the overall performance.
This highlights the advantages of exploiting contextual information among different HOIs.
Performing feature aggregation on \emph{both} subgraphs further improves the final performance.

\para{Effectiveness of each subgraph.}
To validate the effectiveness of the proposed subgraph, we show different variants of our model in~\tabref{ablation}(c).
%
Adding only \emph{human-centric} subgraph improves upon the baseline model (without using any subgraph) by $0.96$ absolute mAP, while adding only \emph{object-centric} subgraph gives a $0.64$ absolute mAP.
More importantly, our results show that the performance gain of each subgraph is complementary to each other.
% 
To further validate the effectiveness of the \emph{object-centric} subgraph, we show in \tabref{ablation}(d) the breakdown of \tabref{ablation}(c) in terms of the number of persons in the scene. The \emph{object-centric} subgraph is less effective for cases with few people. For example, if there is only one person, the \emph{object-centric} subgraph has no effect. For images with a moderate amount of persons (4-6), however, our \emph{object-centric} subgraph shows a clear $0.98$ mAP gain. As the number of persons getting larger (7+), the \emph{object-centric} subgraph shows a relatively smaller improvement due to clutter. Among the 2,867 testing images, 68\% of them have only 1-3 persons. As a result, we do not see significant overall improvement.

\para{Spatial-semantic representation.}
To demonstrate the advantage and effectiveness of the use of the abstract spatial-semantic representation, we show in \tabref{ablation}(b) the comparison with alternative features, e.g., word2vec (as used in \cite{Lu-ECCV-Prior}) or appearance-based features.
By using our spatial-semantic representation in the dual relation graph, we achieve $51.37$ mAP. This shows a clear margin over the other alternative options, highlighting the contribution of spatial-semantic representation.

% \para{Object category representation.}
% \tabref{ablation}(b) compares different ways to represent object category in our spatial-semantic representation. 
% %
% The most straightforward way is to use a one-hot vector (where each entry represents the object class).
% %
% Compared to the baseline where no category is included, using one-hot vector provides sizable improvement. 
% % 
% However, as one-hot vector representation fails to capture the semantic relationships among objects (e.g., riding a \emph{bicycle} may be similar to riding a \emph{motorcycle}), it leads to sub-optimal results. % , which gives a sub-optimal solution.
% %
% Using the word embedding from fastText~\cite{Mikolov-LREC-fastText} to represent the object category performs better.



% \para{Score fusion option.}
% Since each stream predicts a confidence score independently, we explore different ways of fuse the action prediction scores $s^a_{h}$ (from the human stream), $s^a_{o}$ (from the object stream),$s^a_{spH}$ (from the human-centric spatial-semantic stream), and $s^a_{spO}$ (from the object-centric spatial-semantic stream) to obtain the final prediction in \tabref{ablation}(d).
% %
% % We try three variants: 
% % (1) $s^a_{h} + s^a_{o} + s^a_{sp}$,
% % (2) $s^a_{h} * s^a_{o} * s^a_{sp}$,
% % (3) $(s^a_{h} + s^a_{o}) * s^a_{sp}$,
% We try five variants and find that multiplication of all the scores together $s^a_{h}$ $\cdot$ $s^a_{o}$ $\cdot$ ($s^a_{spH}$ $\cdot$ $s^a_{spO}$) leads to the best overall performance. 

% \input{table/VCOCO_ablation}
\input{figure/fig_failure}

\subsection{Limitations}
While we demonstrated improved performance, our model is far from perfect. 
Below, we discuss two main limitations of our approach, with examples in \figref{failure}.
%  and can be improved from the following perspectives.
%
% \vspace{-0.13mm}

First, we leverage the off-the-shelf object detector to detect object instances in an image. 
The object detection does \emph{not} benefit from the rich contextual cues captured by our method.
% The first two examples show that incorrect object detection causes incorrect interaction predictions. 
% \yl{Show visual example?}
% 
We believe that a joint end-to-end training approach may help reduce this type of errors. 

% since the object detector is not trained with our model jointly, it does not benefit from the rich contextual cues. 
% In \figref{failure}, the first two images show the failures caused by incorrect object detection. 
% 
% Training the whole system end-to-end might help reduce this type of error.
%
Second, our model may be confused by plausible spatial configuration and predicts incorrect action. 
%
In the third image, our model predicts that the person is sitting on a bench even though our model confidently predicts this person is standing and catching a Frisbee.
%
Capturing the statistics of co-occurring actions may resolve such mistakes.


% Third, our model may incorrectly group human and object, even with the help of the proposed object-centric subgraph. For instance, in the last image, our model predicts the action of the highlighted person as ride, but associates the action with an incorrect motorcycle.  


% model encodes the relationship between a specific person to all other objects in the scene. 
% However, we do not leverage the contextual cue from \emph{other people}.
% %
% The last two examples show instructive failure cases from this limitation. 
% % 
% For instance, in the last image, our model predicts the action of the highlighted person as ride, but associates the action with an incorrect motorcycle. 
% % 
% In this case, knowing the other person is riding this particular motorcycle could help \emph{explain away} the scene and alleviate such mis-grouping issue (i.e., the model fails to match the person to the correct related object).



% \paragraph{Datasets.}
% % Describe datasets used, statistics (# images, train/test splits)
% %
% \underline{V-COCO} dataset~\cite{Gupta-SemanticRoleLabeling} is constructed by augmenting the COCO dataset~\cite{Lin-ECCV-MSCOCO} with additional human-object interaction annotations.
% %
% V-COCO consists of a total of 10,346 images containing 16,199 human instances. 
% %
% Each person is annotated with a binary label vector for 26 different action categories (where each entry indicates whether the person is performing a certain action). 
% % 
% Each person can perform multiple actions at the same time, e.g., holding a cup while sitting on a chair.
% %
% Three action classes (\texttt{cut}, \texttt{hit}, \texttt{eat}) are annotated with two types of target objects: (1) instrument and (2) direct object.
% %
% For example, \texttt{eat} + \texttt{fork} involves the instrument (meaning ``eat with a fork"), and \texttt{eat} + \texttt{pizza} involves the direct object (meaning `eat a pizza').
% %
% To address this issue, we consider these three actions with different targets as independent actions, resulting in a total of 29 action classes.
% %
% \underline{HICO-DET}~\cite{Chao-CVPR-HICO} is a larger dataset containing 600 HOI categories over 80 object categories (same as \cite{Lin-ECCV-MSCOCO}) with more than 150K annotated instances of human-object pairs.
% %
% % Note: we arrange the dataset a little bit.
% We disentangle the 600 HOI categories into 117 object-agnostic action categories and train our network over these 117 action categories. 
% %
% Later we combine the predicted object-agnostic action and the detected object and convert this action-object back to 600 HOI classes.
% \chen{Mention that we convert the action and object back to 600 HOI classes.}
% As there is no official \emph{validation} set, we randomly sample $10\%$ of the training data and treat them as the held-out \emph{val} set.

==> [ECCV 2020] HOI arXiv/5_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}
% Briefly summarize what we did in this work.
In this paper, we present a Dual Relation Graph network for HOI detection. 
Our core idea is to exploit the \emph{global object layout} as contextual cues and use a \emph{human-centric} as well as an \emph{object-centric} subgraph to propagate and integrate rich relations among individual HOIs.
We validate the efficacy of our approach on two large-scale HOI benchmark datasets and show our model achieves a sizable performance boost over the state-of-the-art algorithms.
We also find that using the abstract spatial-semantic representation alone (i.e., without the appearance features extracted from a deep CNN) yields competitive accuracy, demonstrating a promising path of activity understanding through visual abstraction.

\para{Acknowledgements} We thank the support from Google Faculty Award.

==> [ECCV 2020] HOI arXiv/figure/fig_HCVRD_more.tex <==
\begin{figure*}[t]
\centering

% HCVRD
\mfigure{0.151}{{figure_HCVRD/holds_420_37.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_910_249.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_2333_57.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_3453_4.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_3453_479.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_713118_274.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HCVRD/in_87_494.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_323_499.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_408_369.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_455_273.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_1615_451.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_4587_130.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HCVRD/wearing_3185_156.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_3235_280.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_3548_261.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_4587_180.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_4611_481.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_4982_235.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HCVRD/with_355_513.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_420_37.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_637_302.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_2383_149.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_2870_1.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_713352_22.jpg}}\\
% \vspace{0.5mm}
% \vspace{\figcapmargin}
% \captionof{figure}{\textbf{HOI detection results on the HCVRD \emph{test} set.}}
\caption{\textbf{HOI detection results on HCVRD \emph{test} set.}}
\label{fig:HCVRD_more}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_HICO_more.tex <==
\begin{figure*}[t]
\centering

% HICO
\mfigure{0.151}{{figure_HICO/carry_000000003392_218.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000003535_115.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000006088_103.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000006501_3.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000008037_101.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000008849_414.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/wear_000000000874_52.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000000906_128.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000001045_122.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000001980_253.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000003565_281.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000009605_23.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/board_000000000018_442.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/ride_000000001551_241.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000002640_94.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000004704_211.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000006379_284.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000008525_394.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/eat_000000002327_208.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000004013_200.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000006943_175.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000008015_54.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000008635_104.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000008983_17.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/feed_000000003253_111.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000006182_327.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000006463_4.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000007259_0.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000008156_386.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000008575_2.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/hold_000000000073_125.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000248_250.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000275_130.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000277_19.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000412_99.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000523_2.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/read_000000000412_99.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000002774_354.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000005884_101.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000006963_83.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000007579_245.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000007871_1.jpg}}\\
% \vspace{0.5mm}
% \vspace{\figcapmargin}
% \captionof{figure}{\textbf{More HOI detection results on the HICO-DET \emph{test} set.}}
\caption{\textbf{HOI detection results on HICO-DET \emph{test} set.}}
\label{fig:HICO_more}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_HICO_not_annotated.tex <==
\begin{figure*}[t]
\centering
\newlength\ftsa
\setlength\ftsa{3cm} % page-width size
\newlength\ftsb
\setlength\ftsb{0.0mm}
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002714_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/ride_000000001454_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002464_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/straddle_000000000011_gt.jpg}\vspace{\ftsb}\\%
 Ground truth}%
%
\hfill%
%
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002714_3.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/ride_000000001454_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002464_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/straddle_000000000011_1.jpg}\vspace{\ftsb}\\%
 Our detections}%
%
\hfill%
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002506_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/read_000000000874_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000001297_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/hold_000000001529_gt.jpg}\vspace{\ftsb}\\%
 Ground truth}%
%
\hfill%
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002506_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/read_000000000874_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000001297_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/hold_000000001529_1.jpg}\vspace{\ftsb}\\%
 Our detections}%
\vspace{\figcapmargin}
\caption{\textbf{HICO-DET is not fully annotated.}
The first and third column shows \emph{all} the ground truth annotations. The second and last column shows the HOI detection from our model. While our method correctly detects the HOIs, we are penalized because the dataset is not fully annotated.
}
\label{fig:HICO_not_annotated}
\end{figure*}


% \begin{figure*}[t]
% \centering
% \newlength\ftsa
% \setlength\ftsa{3cm} % page-width size
% \newlength\ftsb
% \setlength\ftsb{0.0mm}
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_sp.png}\vspace{\ftsb}\\%
% \scriptsize Spatial only}%
% %
% \hfill%
% %
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_O.png}\vspace{\ftsb}\\%
% \scriptsize Spatial+ Obj App.}%
% %
% \hfill%
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_onehot.png}\vspace{\ftsb}\\%
% \scriptsize Spatial + One-hot vec.}%
% %
% \hfill%
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_fastText_0.png}\vspace{\ftsb}\\%
% \scriptsize Spatial + fastText}%
% \caption{\textbf{t-SNE visualization of different object category representation.}
% }
% \label{fig:tsne}
% \end{figure*}



==> [ECCV 2020] HOI arXiv/figure/fig_RBG.tex <==
\newlength\ftqd
\setlength\ftqd{1.9cm}
\begin{figure*}[t]
\centering

\mpage{0.01}{\rotatebox[origin=c]{90}{\small Human-centric}}
\mpage{0.95}{
\includegraphics[width=\ftqd]{figure_SSAR/human_000000235316.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000235316_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000235316_cut_plot.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000034837.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000034837_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000034837_lay_plot.png}\hfill
\\
\includegraphics[width=\ftqd]{figure_SSAR/human_000000421491.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000421491_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000421491_hit_plot.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000005689.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000005689_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/human_000000005689_sit_plot.png}\hfill
\\
}
%

\mpage{0.01}{\rotatebox[origin=c]{90}{\small Object-centric}}
\mpage{0.95}{
\includegraphics[width=\ftqd]{figure_SSAR/000000423602_2199.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000423602_2199_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000423602_2199_hold_plot.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000455667_2365.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000455667_2365_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000455667_2365_ride_plot.png}\hfill
\\
\includegraphics[width=\ftqd]{figure_SSAR/000000299932_1487.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000299932_1487_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000299932_1487_kick_plot.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000178874_901.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000178874_901_weight.png}\hfill%
\includegraphics[width=\ftqd]{figure_SSAR/000000178874_901_work_on_computer_plot.png}\hfill
\\
}
%

% \mpage{0.04}{}\hfill
% \mpage{0.92}{
% \mpage{0.14}{HOI det.} \hfill
% \mpage{0.14}{H-O pair} \hfill
% \mpage{0.14}{Score} \hfill
% \mpage{0.14}{HOI det.} \hfill
% \mpage{0.14}{H-O pair} \hfill
% \mpage{0.14}{Score}
% }
\mpage{0.04}\hfill
\mpage{0.13}{HOI det.} \hfill
\mpage{0.13}{H-O pair} \hfill
\mpage{0.13}{Score} \hfill
\mpage{0.13}{HOI det.} \hfill
\mpage{0.14}{H-O pair} \hfill
\mpage{0.13}{Score}\hfill
% \\
% \underbracket[1pt][2.0mm]{\hspace{\textwidth}}_%
%     {\substack{\vspace{-3.0mm}\\\colorbox{white}{~~Our results~~}}}
\\
\mpage{0.015}\hfill
\mpage{0.46}{
% Increasing scores for correct pairs
$\underbracket[1pt][2.0mm]{\hspace{\textwidth}}_
    {\substack{\vspace{-1.0mm}\\\colorbox{white}{~~Increasing scores for correct HOIs~~}}}$
}\hfill
\mpage{0.485}{
% Suppressing scores for unrelated pairs
$\underbracket[1pt][2.0mm]{\hspace{\textwidth}}_
    {\substack{\vspace{-1.0mm}\\\colorbox{white}{Suppressing scores for unrelated pairs}}}$
}\hfill
\caption{\textbf{More iteration of feature aggregation leads to a more accurate prediction.} 
The human-centric and object-centric subgraph in the spatial-semantic stream propagates contextual information to produce increasingly accurate HOI predictions.
}
\label{fig:RBG}
\end{figure*}

\vspace{1.0mm}

==> [ECCV 2020] HOI arXiv/figure/fig_Tsne.tex <==
\begin{figure*}[t]
\centering
% \newlength\ftsa
\setlength\ftsa{3cm} % page-width size
% \newlength\ftsb
\setlength\ftsb{0.0mm}
\parbox[t]{\ftsa}{
\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_sp.png}\\%
\scriptsize Spatial only}%
%
\hfill%
%
\parbox[t]{\ftsa}{\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_O.png}\\%
\scriptsize Spatial+ Obj App.}%
%
\hfill%
\parbox[t]{\ftsa}{\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_onehot.png}\\%
\scriptsize Spatial + One-hot vec.}%
%
\hfill%
\parbox[t]{\ftsa}{\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_fastText_0.png}\\%
\scriptsize Spatial + fastText}%
\caption{\textbf{t-SNE visualization of different object category representation.}
}
\label{fig:tsne}
\end{figure*}



==> [ECCV 2020] HOI arXiv/figure/fig_Tsne_DRG.tex <==
\begin{figure*}[t]
\centering

\newlength\ffca
\setlength\ffca{4cm} % page-width size
\newlength\ffcb
\setlength\ffcb{-0.0mm}

\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/Tsne_fastText_0.png}\\%
 Human-centric 0 iter.}%
%
\hfill%
%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/Tsne_fastText_1.png}\\%
 Human-centric 1 iter.}%
%
\hfill%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/Tsne_fastText_2.png}\\%
 Human-centric 2 iter.}%
%
\hfill%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/tsne_object_centric_0.png}\\%
 Object-centric 0 iter.}%
%
\hfill%
%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/tsne_object_centric_1.png}\\%
 Object-centric 1 iter.}%
%
\hfill%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/tsne_object_centric_2.png}\\%
 Object-centric 2 iter.}%
\mfigure{0.7}{{fig/color_bar.png}}\\
\vspace{2mm}
\caption{\textbf{t-SNE visualization of spatial-semantic representation with different iterations of feature aggregation.}
}
\label{fig:tsne_DRG}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_VCOCO_more.tex <==
\begin{figure*}[t]
\centering

% V-COCO
\mfigure{0.151}{{figure_VCOCO/carry_000000301867_251.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000550714_0.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000144863_0.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000543570_199.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hold_000000012991_50.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hold_000000427615_170.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/ski_000000010142_320.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/snowboard_000000149014_198.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000062363_367.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/talk_000000263351_5.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/skateboard_000000541017_43.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/jump_000000186721_351.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/catch_000000015846_197.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/cut_000000091318_4.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000121442_282.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000003716_218.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hold_000000032334_96.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/kick_000000282225_328.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/hold_000000256983_141.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000310035_341.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000032300_167.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000186711_298.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/work_000000086011_44.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000087740_119.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/look_000000153717_329.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000276024_237.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000504353_84.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/throw_000000404517_57.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000413044_113.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/kick_000000204137_280.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/sit_000000223414_216.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/carry_000000247264_422.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/cut_000000012991_50.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/skateboard_000000412975_1.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000437540_375.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/throw_000000072376_264.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/cut_000000314074_0.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000358231_267.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000180764_2.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/sit_000000526904_91.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000432623_350.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000137297_134.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/hit_000000306335_265.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/snowboard_000000001700_212.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000032300_305.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000276893_202.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000106617_1.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000509471_178.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/work_000000526904_91.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000543570_253.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ski_000000341719_320.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000567494_247.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000204432_122.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/sit_000000577614_400.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/talk_000000528729_169.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000295316_189.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/snowboard_000000564743_227.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ski_000000346589_90.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000485673_125.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000480408_117.jpg}}
\\
\caption{\textbf{HOI detection results on V-COCO \emph{test} set.}}
\label{fig:VCOCO_more}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_bipartite.tex <==
\begin{figure}[t]
% \includegraphics[width=\linewidth]{fig/Bipartite_v3.pdf}
\includegraphics[width=\linewidth]{fig/Bipartite_v4.pdf}
\caption{\textbf{HOI detection using Dual Relation Graph.} 
% 
(a) The input to our model are the detected objects in the given image. 
We denote $\mathbb{H}$ as the set of human detections, and $\mathbb{O}$ as the set of object detections.
% 
(b) We construct a \emph{relation graph} from the detections where the two sets are  $\mathbb{H}$ and $\mathbb{O}$.
% 
(c) For each human node \textit{h} in $\mathbb{H}$, we obtain a human-centric sub-graph where all nodes in $\mathbb{O}$ are connected to \textit{h}. 
Similarly, we can obtain an object-centric sub-graph for each object node \textit{o} in $\mathbb{O}$. 
Note that ``person'' is also an object category. 
For simplicity, we do not show it in the figure.
% 
(d) In order to predict HOIs, we need to construct the HOI graph explicitly. 
Taking human sub-graph for example, we insert an HOI node \textit{x} between human node \textit{h} and object node \textit{o}. 
We then connect all the HOI nodes and obtain the \textit{human-centric} HOI sub-graph and the \textit{object-centric} HOI sub-graph.
% 
(e) We iteratively update the HOI node feature via a trainable attentional graph convolutional network. 
This helps to aggregate the contextual information. 
% 
(f) We fuse the scores from both sub-graphs and make the final HOI prediction.
% \chen{How to name Fig 4b? We could not call it Dual graph here.}
% \yl{I think we can just name it bipartite graph, which it indeed is.}
}
\label{fig:bipartite_graph}
\end{figure}
% 

==> [ECCV 2020] HOI arXiv/figure/fig_error.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}{0.45\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/iCAN_error.pdf}}
\end{minipage}
%
\hfill
\begin{minipage}{0.45\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/DRG_error.pdf}}
\end{minipage}
\hfill
\begin{minipage}{0.07\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/Legend.pdf}}
\end{minipage}
\\
\mpage{0.48}{(a) iCAN} \hfill
\mpage{0.48}{(b) DRG} \hfill
\\
\captionof{figure}{
\textbf{Comparison of the distribution of the error categories between iCAN and our proposed DRG.} We show the distribution of the incorrect detections for each action class. \tb{`incorrect label'} refers to the detected person is predicted to perform an action which he does not. \tb{`bck'} indicates the object detector fails to localize the person (IoU with any ground truth person is less than 0.1). \tb{`person misloc'} means the detected person is not localized well (IoU is between $0.1$ and $0.5$ with a ground truth person) regardless of the related object. \tb{`object misloc'} refers to the detected object is not localized well while the related person is successfully localized. \tb{`mis-grouping'} indicates the person is successfully localized, but the network fails to match the person to the correct related object (IoU between the ground truth associated object and the predicted object is less than 0.1). \tb{`occlusion'} means we incorrectly associate an object with a correct detected person, while the object is not annotated in the ground truth due to occlusions.
%
\tb{Discussion:} our proposed DRG helps most with the mis-grouping. By leveraging the proposed human-centric subgraph and object-centric subgraph, we can enhance the correct HOIs and suppress the unrelated pairs. As a result, the mis-grouping error is reduced, especially for the action classes that humans and objects have a typical spatial relationship, \eg $\textit{hit obj}$, $\textit{hit instr}$, and $\textit{skateboard instr}$.
}
\label{fig:error}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_failure.tex <==
\begin{figure*}[!t]
\centering
% \mfigure{0.145}{{figure_failure/incorrect_obj_ski_000000110769_71.jpg}}\hfill
% \mfigure{0.145}{{figure_failure/incorrect_obj_talk_000000020925_49.jpg}}\hfill
% \mfigure{0.145}{{figure_failure/incorrect_action_sit_000000015846_212.jpg}}\hfill
% \mfigure{0.145}{{figure_failure/incorrect_action_mcarry_000000191314_255.jpg}}\hfill
% \mfigure{0.145}{{figure_failure/mis_group_hold_000000417632_343.jpg}}\hfill
% \mfigure{0.145}{{figure_failure/mis_group_ride_000000204906_418.jpg}}\hfill
% \\
\includegraphics[width=\ftqa]{figure_failure/incorrect_obj_ski_000000110769_71.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_failure/incorrect_obj_talk_000000020925_49.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_failure/incorrect_obj_sit_000000472256_206.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_failure/incorrect_action_sit_000000015846_212.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_failure/incorrect_action_mcarry_000000191314_255.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_failure/incorrect_action_sit_000000032334_96.jpg}%
%
\mpage{0.45}{Incorrect object} \hfill
\mpage{0.45}{Incorrect action}
\caption{
%
\textbf{Failure cases of our method.}
}
\label{fig:failure}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_failure_more.tex <==
\begin{figure*}[t]
\centering
\mfigure{0.155}{{figure_failure/incorrect_obg_look_000000072376_264.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_obj_hit_000000375021_160.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_ride_000000424464_48.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_ride_000000171548_307.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_work_000000149783_220.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_eat_000000023807_233.jpg}}\hfill
\\
\mfigure{0.155}{{figure_failure/incorrect_obj_sit_000000472256_206.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_obj_eat_000000041279_45.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_skateboard_000000002179_220.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_sit_000000032334_96.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_sit_000000025603_338.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_ride_000000370657_404.jpg}}\hfill
\\

\mpage{0.31}{Incorrect object} \hfill
\mpage{0.31}{Incorrect action} \hfill
\mpage{0.31}{Mis-grouping}
\caption{
%
\textbf{More failure cases.} 
}
\label{fig:failure_more}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_module.tex <==
\begin{figure*}[t]
\includegraphics[width=\linewidth]{fig/SSAR.pdf}
\caption{
%
\textbf{SSAR module.} To recognize the interaction between the $i$-th person and the $j$-th object, we first pair the $i$-th person with all $N$ objects in an image. Given the spatial relation between the $i$-th person and the $j$-th object, as well as the word embedding of the $j$-th object's category, we generate a spatial-semantic representation $\mathbf{x}_{i,j}$ by concatenating the convolved $64 \times 64 \times 2$ spatial pattern with the $300D$ word embedding vector.
%
We aggregate all the spatial-semantic features which involved the same person, \ie $\{\mathbf{x}_{i, j^\prime}| j^\prime \in \{1 \cdots N\}\}$, to obtain the aggregated spatial-semantic features $\mathbf{x}_{i, j}^{\prime\prime}$.
%
\ignorethis{
We use the linear transformation $W_Q$ and $W_K$ to generate the query $\mathbf{q}_{i, j}$ and key $\mathbf{k}_{i, j^\prime}$. 
%
We obtain the attention weights by performing the scaled dot-product attention of the query over the key features. 
%
The spatial-semantic representation $\mathbf{x}_{i, j}^\prime$ is an attentioal weighted sum of all spatial-semantic representations of this person, transformed by $W_V$.
%
We apply a dropout to $\mathbf{x}_{i, j}^\prime$ and add it to the original feature $\mathbf{x}_{i, j}$.
%
We finally pass $\mathbf{x}_{i, j}^\prime$ through LayerNorm and yield the aggregated feature $\mathbf{x}_{i, j}^{\prime\prime}$. 
}
%
% We use $\mathbf{x}_{i, j}^{(0)}$ to denote the initial spatial-semantic feature. We use $\mathbf{x}_{i, j}^{(k)}$ to denote the aggregated feature after $k$ SSAR module.
}
\label{fig:module}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_motivation.tex <==
\newlength\ffma
\setlength\ffma{3cm} % page-width size
\newlength\ffmb
\setlength\ffmb{-0.0mm}

\begin{figure}[t]
\centering%

\parbox[t]{\ffma}{
\centering%
\includegraphics[width=\ffma]{fig/Motivation_1.pdf}\\%
 \tiny (a) Object detection}%
%
\hfill%
%
\parbox[t]{\ffma}{
\centering%
\includegraphics[width=\ffma]{fig/Motivation_indep.pdf}\\%
 \tiny (b) Independent}%
%
\hfill%
\parbox[t]{\ffma}{
\centering%
\includegraphics[width=\ffma]{fig/Motivation_full.pdf}\\%
 \tiny (c) Densely connected}%
%
\hfill%
\parbox[t]{\ffma}{
\centering%
\includegraphics[width=\ffma]{fig/Motivation_ours.pdf}\\%
 \tiny (d) Ours (human-centric)}%

  \captionof{figure}{
\textbf{Leveraging contextual information.} Given object detections in the scene (a), existing HOI detection algorithms only perform \emph{independent} prediction for each Human-object pair (b), ignoring the rich contextual cues. Recent methods in visual relationship detection (or scene graph generation) perform \emph{joint inference} on a densely connected graph (c). While being general, the large number of relations among the dense connections makes the learning and inference on such a graph challenging. 
In contrast, our work leverages the human/object-centric graph to focus only on relevant contexts for improved HOI detection (d). 
}
  \label{fig:motivation}
\end{figure}


==> [ECCV 2020] HOI arXiv/figure/fig_multi_action.tex <==
\begin{figure}[t]
\centering
\mfigure{0.32}{figure_multi_action/eat_000000146120_273_1.jpg}\hfill
\mfigure{0.32}{figure_multi_action/hold_000000146120_273_3.jpg}\hfill
\mfigure{0.32}{figure_multi_action/sit_000000146120_273_2.jpg}
% \\
% \mfigure{0.32}{figure_multi_action/eat_000000132272_173_1.jpg}\hfill
% \mfigure{0.32}{figure_multi_action/hold_000000132272_173_3.jpg}\hfill
% \mfigure{0.32}{figure_multi_action/drink_000000132272_173_2.jpg}
\\
\caption{
\textbf{Detecting multiple actions.} Our model can detect a person doing different actions with different objects.
}
\label{fig:multi_action}
\end{figure}

==> [ECCV 2020] HOI arXiv/figure/fig_multi_action_more.tex <==
\begin{figure*}[t]
\centering
\mfigure{0.152}{{figure_multi_action/hold_000000007298_183_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/catch_000000007298_183_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000007298_183_3.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/sit_000000577614_400_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000577614_400_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/work_000000577614_400_3.jpg}}\hfill
\\
\mfigure{0.152}{{figure_multi_action/hold_000000567494_247_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/hit_000000567494_247_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000567494_247_3.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/sit_000000300330_70_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000300330_70_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/work_000000300330_70_3.jpg}}\hfill
\\
\caption{
\textbf{Detecting multiple actions.} Our model can detect a person doing different actions with different objects. 
}
\label{fig:multi_action_more}
\end{figure*}

==> [ECCV 2020] HOI arXiv/figure/fig_overview.tex <==
\begin{figure}[t]
\includegraphics[width=\linewidth]{fig/Overview.pdf}
\caption{\textbf{Overview of the proposed model.} 
Our network consists of three streams (human, object, and spatial-semantic).
%
The human and object stream leverage the appearance feature $\mathbf{f}_h$ and $\mathbf{f}_o$.
%
The spatial-semantic stream makes a prediction from the abstract spatial-semantic feature $\bold{x}$. 
%
We apply our proposed dual relation graph (DRG) to this stream. 
%
The three streams predict the scores $s_h^a$, $s_o^a$, $s_{spH}^a$ and $s_{spO}^a$, which are fused to form final prediction.
}
\label{fig:overview}
\end{figure}

==> [ECCV 2020] HOI arXiv/figure/fig_teaser.tex <==
\newlength\ffca
\setlength\ffca{4cm} % page-width size
\newlength\ffcb
\setlength\ffcb{-0.0mm}

\begin{center}
  %
\parbox[t]{\ffca}{
\centering%
\includegraphics[width=\ffca]{fig/Teaser_det.pdf}\\%
 (a) Object detection}%
%
\hfill%
%
\parbox[t]{\ffca}{
\centering%
\includegraphics[width=\ffca]{fig/Teaser_H_v1.pdf}\\%
 (b) Human-centric}%
%
\hfill%
\parbox[t]{\ffca}{
\centering%
\includegraphics[width=\ffca]{fig/Teaser_O_v1.pdf}\\%
(c) Object-centric}%

  \captionof{figure}{
    \textbf{Human-object interaction (HOI) detection using dual relation graph.}
    %
    Predicting each HOI in isolation is ambiguous due to the lack of context. 
    In this work, we propose to leverage a dual relation graph. 
    % There are two types of nodes, $\mathbb{H}$ and $\mathbb{O}$.
    % 
    For each human node \textit{h}, we obtain a \emph{human-centric} subgraph where all object nodes are connected to \textit{h}.
    %
    Similarly, we can obtain an \emph{object-centric} subgraph for each object node \textit{o}.
    % The bipartite graph can be divided into a human sub-graph and an object sub-graph.
    %
    The human subgraph helps to adjust single HOI's prediction based on the same person's other HOIs. For example, knowing a 
    \textbf{\textcolor[HTML]{ff1744}{person}} 
    is wearing a 
    \textbf{\textcolor[HTML]{ff9900}{baseball helmet}}
    and hitting a 
    \textbf{\textcolor[HTML]{dfcf44}{baseball}} 
    suggests that the 
    \textbf{\textcolor[HTML]{ff1744}{person}} 
    may be holding a 
    \textbf{\textcolor[HTML]{38761d}{baseball bat}}.
    %
    Similarly, the object subgraph helps to refine the HOI's prediction based on other HOIs associated with the same object. 
    For example, knowing a 
    \textbf{\textcolor[HTML]{38761d}{baseball bat}} 
    is held by a 
    \textbf{\textcolor[HTML]{ff1744}{person}} 
    lowers the chance that it is held by another 
    \textbf{\textcolor[HTML]{00ffff}{person}}.
    %
    Our method exploits such cues for improving HOI detection.
  }
  \label{fig:teaser}
\end{center}

% \textcolor[HTML]{ffeb3b}{yellow}
% \textcolor[HTML]{ff1744}{red}
% \textcolor[HTML]{00ffff}{cyan}
% \textcolor[HTML]{38761d}{green}
% \textcolor[HTML]{ff9900}{orange}


==> [ECCV 2020] HOI arXiv/figure/fig_visual.tex <==
\newlength\ftqa
\setlength\ftqa{2.0cm}
\newlength\ftqb
\setlength\ftqb{0.2mm}
\newlength\ftqc
\setlength\ftqc{0.8mm}

\begin{figure*}[t]

\includegraphics[width=\ftqa]{figure_VCOCO/look_000000153717_329.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_VCOCO/eat_000000550714_0.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_VCOCO/eat_000000144863_0.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_VCOCO/hit_000000543570_199.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_VCOCO/hold_000000012991_50.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_VCOCO/hold_000000427615_170.jpg}\vspace{\ftqb}\\%
%
% \includegraphics[width=\ftqa]{figure_VCOCO/lay_000000216326_29.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_VCOCO/look_000000003716_218.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_VCOCO/ride_000000016961_144.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_VCOCO/carry_000000301867_251.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_VCOCO/sit_000000292463_78.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_VCOCO/skateboard_000000541017_43.jpg}\vspace{\ftqb}\\%
%
\includegraphics[width=\ftqa]{figure_HICO/ride_000000003622_257.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_HICO/ride_000000006887_149.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_HICO/ride_000000007873_207.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_HICO/ride_000000001551_241.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_HICO/ride_000000003086_218.jpg}\hfill%
\includegraphics[width=\ftqa]{figure_HICO/ride_000000005048_214.jpg}%\vspace{\ftqb}\\%
%
% \includegraphics[width=\ftqa]{figure_HICO/carry_000000003392_218.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_HICO/carry_000000003535_115.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_HICO/carry_000000006088_103.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_HICO/carry_000000006501_3.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_HICO/carry_000000008037_101.jpg}\hfill%
% \includegraphics[width=\ftqa]{figure_HICO/carry_000000008849_414.jpg}%
%
\caption{\textbf{Sample HOI detections on V-COCO (first row) and HICO-DET (second row) \emph{test} set.}
\label{fig:visual}
}
\end{figure*}
\vspace{-3.0mm}
% \begin{figure*}[t]
% \centering

% \mfigure{0.151}{{figure_VCOCO/look_000000153717_329.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/eat_000000550714_0.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/eat_000000144863_0.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/hit_000000543570_199.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/hold_000000012991_50.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/hold_000000427615_170.jpg}}\hfill
% \\
% \vspace{0.5mm}
% \hfill
% \mfigure{0.151}{{figure_VCOCO/lay_000000216326_29.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/look_000000003716_218.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/ride_000000016961_144.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/carry_000000301867_251.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/sit_000000292463_78.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/skateboard_000000541017_43.jpg}}\hfill
% \\
% \vspace{0.5mm}
% \hfill
% \mfigure{0.151}{{figure_HICO/ride_000000003622_257.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000006887_149.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000007873_207.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000001551_241.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000003086_218.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000005048_214.jpg}}\hfill
% \\
% \vspace{0.5mm}
% \hfill
% \mfigure{0.151}{{figure_HICO/carry_000000003392_218.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/carry_000000003535_115.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/carry_000000006088_103.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/carry_000000006501_3.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/carry_000000008037_101.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/carry_000000008849_414.jpg}}\hfill
% \\
% \vspace{\figcapmargin}
% \caption{\textbf{Sample HOI detections on V-COCO (first row) and HICO-DET (second row) \emph{test} set.}
% }
% \label{fig:visual}
% \end{figure*}

% \begin{figure*}[t]
% \centering

% % V-COCO
% \mfigure{0.151}{{figure_VCOCO/look_000000153717_329.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/eat_000000550714_0.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/eat_000000144863_0.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/hit_000000543570_199.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/hold_000000012991_50.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/hold_000000427615_170.jpg}} \\
% \vspace{0.5mm}
% \mfigure{0.151}{{figure_VCOCO/lay_000000216326_29.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/look_000000003716_218.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/ride_000000016961_144.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/carry_000000301867_251.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/sit_000000292463_78.jpg}}\hfill
% \mfigure{0.151}{{figure_VCOCO/skateboard_000000541017_43.jpg}} \\
% \vspace{0.5mm}
% % \mfigure{0.151}{{figure_VCOCO/ski_000000010142_320.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/snowboard_000000149014_198.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/surf_000000062363_367.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/talk_000000263351_5.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/throw_000000072376_264.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/jump_000000186721_351.jpg}} \\
% % \vspace{0.5mm}
% % \mfigure{0.151}{{figure_VCOCO/catch_000000015846_197.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/cut_000000091318_4.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/eat_000000121442_282.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/hit_000000306335_265.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/hold_000000032334_96.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/kick_000000282225_328.jpg}} 
% % \\
% % \vspace{0.5mm}
% % \mfigure{0.151}{{figure_VCOCO/hold_000000256983_141.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/lay_000000310035_341.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/look_000000032300_167.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/surf_000000186711_298.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/work_000000086011_44.jpg}}\hfill
% % \mfigure{0.151}{{figure_VCOCO/ride_000000087740_119.jpg}}\\
% % \vspace{0.5mm}
% %
% \mfigure{0.151}{{figure_HICO/ride_000000003622_257.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000006887_149.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000007873_207.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000001551_241.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000003086_218.jpg}}\hfill
% \mfigure{0.151}{{figure_HICO/ride_000000005048_214.jpg}}\\
% \vspace{0.5mm}
% % \mfigure{0.151}{{figure_HICO/carry_000000003392_218.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/carry_000000003535_115.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/carry_000000006088_103.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/carry_000000006501_3.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/carry_000000008037_101.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/carry_000000008849_414.jpg}}\\
% % \vspace{0.5mm}
% % \mfigure{0.151}{{figure_HICO/wear_000000000874_52.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/wear_000000000906_128.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/wear_000000001045_122.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/wear_000000001980_253.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/wear_000000003565_281.jpg}}\hfill
% % \mfigure{0.151}{{figure_HICO/wear_000000009605_23.jpg}}\\
% % \vspace{0.5mm}
% \vspace{\figcapmargin}
% \captionof{figure}{\textbf{Sample HOI detections on V-COCO (first two rows) and HICO-DET (last row) \emph{test} set.
% }
% %Our model is able to detection diverse HOIs from daily images.
% }
% \label{fig:visual}
% \end{figure*}


==> [ECCV 2020] HOI arXiv/setup/graphicspath.tex <==
\graphicspath{{figure}, {example}}


==> [ECCV 2020] HOI arXiv/setup/macros.tex <==
% Macros - Jia-Bin Huang (jbhuang@vt.edu)

\renewcommand{\baselinestretch}{1}       % for squeezing the draft into the page limit, do not use

% =========================================
% Useful macros
% =========================================

% Latin abbreviations
\def\etal{et~al.}			  % and others, and co-workers
\def\eg{e.g.,~}               % for example
\def\ie{i.e.,~}               % that is, in other words
\def\etc{etc}                 % and other things, and so forth
\def\cf{cf.~}                 % compare
\def\viz{viz.~}               % namely, precisely
\def\vs{vs.~}                 % against

\newcommand{\para}[1]{\vspace{1mm}\noindent\textbf{#1}}

% Math related
\DeclareMathOperator*{\argmin}{\arg\!\min} 
\DeclareMathOperator*{\argmax}{\arg\!\max}

% Consistent margin adjustment for paragraphs, figures, and sections
\newlength\paramargin
\newlength\figmargin
\newlength\secmargin
\newlength\figcapmargin
\newlength\tabmargin

\setlength{\secmargin}{0.0mm}
\setlength{\paramargin}{0.0mm}
\setlength{\tabmargin}{0.0mm}
\setlength{\figmargin}{0.0mm}
\setlength{\figcapmargin}{0.0mm}


\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\yellow}{\textcolor{yellow}}
\newcommand{\orange}{\textcolor{orange}}
\newcommand{\green}{\textcolor{green}}

\newcommand {\first}[1]{{\color{red}\textbf{#1}}}
\newcommand {\second}[1]{{\color{blue}\underline{#1}}}


% minipage
\newcommand{\mpage}[2]
{
\begin{minipage}{#1\linewidth}\centering
#2
\end{minipage}
}

% mini-figure
\newcommand{\mfigure}[2]
{
\begin{subfigure}{#1\linewidth}\centering
\includegraphics[width=\linewidth]{#2}
\end{subfigure}
}



% heading (replace \paragraph)
\newcommand{\heading}[1]
{
\vspace{1mm}\noindent\textbf{#1}
}


% References for figures, tables, equations, and sections
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}} 
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\prgref}[1]{Program~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\clmref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\ptyref}[1]{Property~\ref{#1}}

% Comments
\long\def\ignorethis#1{}

% \ignorethis{
\newcommand {\jiabin}[1]{{\color{magenta}\textbf{Jia-Bin: }#1}\normalfont}
\newcommand {\chen}[1]{{%
\color{red}\textbf{C}%
\color{red}\textbf{h}%
\color{red}\textbf{e}%
\color{red}\textbf{n}%
\color{red}\textbf{: }%
\color{red} #1}\normalfont\xspace}
\newcommand {\todo}{{\textbf{\color{red}[TO-DO]\_}}}
\def\newtext#1{\textcolor{blue}{#1}}
\def\modtext#1{\textcolor{red}{#1}}
% \newcommand{\note}[1]{{\it\color{blue} #1}}
% }
\newcommand {\yl}[1]{{\color{red}\textbf{YL: }#1}\normalfont}
\newcommand {\jiarui}[1]{{\color{blue}\textbf{Jiarui: }#1}\normalfont}

\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}

\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}

\newcommand{\jblock}[2]{%
	\begin{minipage}[t]{#1}\vspace{0cm}\centering%
	#2%
	\end{minipage}%
}

\makeatletter
\newenvironment{jalgo}[1][htbp]
  {\renewcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \begin{minipage}{\dimexpr\columnwidth\relax}
  \setlength{\algowidth}{\hsize}%
%  \setlength{\algowidth}{\dimexpr\columnwidth+\marincrease}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
%  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
  }%
\renewcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{minipage}
  \end{lrbox}%
  \makebox[\linewidth][c]{\algocf@makethealgo}% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
  \begin{algorithm}[#1]}
  {\end{algorithm}}
\makeatother




==> [ECCV 2020] HOI arXiv/setup/package.tex <==

% Figures
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
%\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{lscape}     % Useful for wide tables or figures.


% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{paralist}
\usepackage{enumitem}

% Math
\usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
\usepackage{graphicx}                  % another package that works for figures
%\usepackage{times}
%\usepackage{mathptmx}
\usepackage{mathtools}

% Fonts
%\usepackage{units}
\usepackage{color}

% Comments
\usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
%\usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}
\usepackage[pagebackref=false,breaklinks=true,colorlinks=true,filecolor=blue,urlcolor=blue,linkcolor=red,bookmarks=false]{hyperref}
% \usepackage[pagebackref=false,breaklinks=true,colorlinks=true,filecolor=blue,urlcolor=blue,citecolor=blue,linkcolor=red,bookmarks=false]{hyperref}
\usepackage[nocompress]{cite}

\usepackage{listings}

% \usepackage{slashbox}
\usepackage{xspace}
\usepackage[table]{xcolor}
\usepackage{setspace}

\usepackage{nicefrac}
\usepackage{microtype}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese


==> [ECCV 2020] HOI arXiv/setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}


==> [ECCV 2020] HOI arXiv/table/HCVRD_results.tex <==
\begin{table}[t]
\centering
\caption{\tb{Performance comparison with the state-of-the-art on the HCVRD $\emph{test}$ set.} The performance is measured by Recall@50 (R@50) and Recall@100  (R@100) under two different settings, namely top-1 and top-3. The best performance is in \first{bold} and the second best is \second{underscored}. Character $^\star$ indicates that the results are reported by \cite{wang2019deep}.
}
\label{tab:HCVRD_comparison}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lc|cc|cc}
\toprule
       &                  & \multicolumn{4}{c}{Predicate Det.} \\
Method & Feature backbone & \multicolumn{2}{c}{R@50} & \multicolumn{2}{c}{R@100} \\
       &                  & top-1 & top-3 & top-1 & top-3 \\
\midrule
Multilabel~\cite{Zhuang-AAAI-HCVRD}         & VGG-16     & 0.9  & 2.8  & 0.9  & 2.8  \\
JointCNN~\cite{Zhuang-AAAI-HCVRD}           & VGG-16     & 2.7  & 7.4  & 2.7  & 7.4  \\
SeparateCNN~\cite{Zhuang-AAAI-HCVRD}        & VGG-16     & 29.0 & 44.4 & 29.0 & 45.9 \\
Webly-Supervised~\cite{Zhuang-AAAI-HCVRD}   & VGG-16     & 31.1 & 47.7 & 31.1 & 49.0 \\
iCAN$^\star$~\cite{Gao-BMVC-iCAN} & ResNet-50 & 33.8 &  48.9 & 33.8 & 49.4 \\
Wang et al. ~\cite{wang2019deep}            & ResNet-50  & 37.1 & 51.3 & 37.1 & 51.9 \\
% \midrule
Ours (S-S only)                             & -          & \second{38.1} & \second{61.8} & \second{38.1} & \second{62.2} \\
% Ours                                        & VGG-16 & - & - & - & - \\
Ours                                        & ResNet-50-FPN & \first{43.6} & \first{65.5} & \first{43.6} & \first{65.9} \\
\bottomrule
\end{tabular}
% }
\end{table}


% Multilabel~\cite{Zhuang-AAAI-HCVRD}         & VGG-16     & 0.9  & 2.8  & 0.9  & 2.8  \\
% JointCNN~\cite{Zhuang-AAAI-HCVRD}           & VGG-16     & 2.7  & 7.4  & 2.7  & 7.4  \\
% SeparateCNN~\cite{Zhuang-AAAI-HCVRD}        & VGG-16     & 29.0 & 44.4 & 29.0 & 45.9 \\
% Webly-Supervised~\cite{Zhuang-AAAI-HCVRD}   & VGG-16     & 31.1 & 47.7 & 31.1 & 49.0 \\
% \midrule
% Ours (S-S only)                              & -             & \textbf{46.4} & \underline{65.3} & \textbf{46.4} & \underline{65.8} \\
% Ours                             & ResNet-50-FPN  & \textbf{46.4} & \textbf{65.6} & \textbf{46.4} & \textbf{66.0} \\

==> [ECCV 2020] HOI arXiv/table/HICO_Resnet50_results.tex <==
\begin{table*}[t]
\centering
\caption{\tb{Results with different feature backbone on the HICO-DET $\emph{test}$ set.}
For the object detector, ``COCO'' means that the detector is trained on COCO, while ``HICO-DET'' means that the detector is first pre-trained on COCO and then further fine-tuned on HICO-DET.
}
\label{tab:HICO_Resnet50}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l cc l ccc c  ccc}
\toprule
\multirow{4}{*}{} & &&&
\multicolumn{3}{c}{Default} & &
\multicolumn{3}{c}{Known Object}\\
\cline{5-7} \cline{9-11}
Method & Detector & Use human pose & Feature backbone & Full & Rare & Non Rare &  & Full & Rare & Non Rare  \\
\midrule
Ours  & COCO & -   & ResNet-50     & 18.87 & 16.90  & 19.45 & & 22.83 & 20.61 & 23.49 \\
Ours & COCO & - &  ResNet-50-FPN & 19.26 & 17.74 & 19.71 & & 23.40 & 21.75 & 23.89 \\ 
\midrule
Ours & HICO-DET & - &  ResNet-50 & 24.05 & 18.72 & 25.65 &  & 27.39 & 22.01 & 28.99 \\
Ours & HICO-DET & - &  ResNet-50-FPN & 24.53 & 19.47 & 26.04 &  & 27.98 & 23.11 & 29.43 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> [ECCV 2020] HOI arXiv/table/HICO_results.tex <==
\begin{table*}[t]
\centering
\caption{\tb{Comparison with the state-of-the-art on HICO-DET \emph{test} set.} The best performance is in \first{bold} and the second best is \second{underscored}. Character $^\star$ indicates that the method uses both VCOCO and HICO-DET training data.
%
For the object detector, ``COCO'' means that the detector is trained on COCO, while ``HICO-DET'' means that the detector is first pre-trained on COCO and then further fine-tuned on HICO-DET.
}
\label{tab:HICO}
\resizebox{\columnwidth}{!}{

\begin{tabular}{l cc l ccc c  ccc}
\toprule
\multirow{4}{*}{} & &&&
\multicolumn{3}{c}{Default} & &
\multicolumn{3}{c}{Known Object}\\
\cline{5-7} \cline{9-11}
Method & Detector & Use human pose & Feature backbone & Full & Rare & Non Rare &  & Full & Rare & Non Rare  \\
\midrule
Shen~\etal~\cite{Shen-WACV-Zeroshot} & COCO & - & VGG-19 & 6.46 & 4.24 & 7.12 & & - & - & -\\
HO-RCNN~\cite{Chao-WACV-HOI} & COCO & - & CaffeNet & 7.81 & 5.37 & 8.54 & & 10.41 & 8.94 & 10.85\\
InteractNet~\cite{Gkioxari-CVPR-InteractNet} & COCO & - & ResNet-50-FPN & 9.94 & 7.16 & 10.77 & & - & - & -\\
GPNN~\cite{Qi-ECCV-GraphParsing} & COCO & - & ResNet-101 & 13.11 & 9.34 & 14.23 &  & - & - & - \\
iCAN~\cite{Gao-BMVC-iCAN} & COCO & - & ResNet-50 & 14.84 & 10.45 & 16.15 & & 16.26 & 11.33 & 17.73 \\
Wang et al.~\cite{wang2019deep} & COCO & - & ResNet-50 & 16.24 & 11.16 & 17.75 && 17.73 & 12.78 & 19.21 \\
Bansal~\etal~\cite{bansal2019detecting} & COCO & - &  ResNet-101 & 16.96 & 11.73 & 18.52 &  & - & - & - \\
$RP_DC_D$~\cite{Li-CVPR-Interactiveness} & COCO & \checkmark & ResNet-50 & 17.03 & 13.42 & 18.11 &  & 19.17 & 15.51 & 20.26 \\
${RP_{T2}C_D}^\star$~\cite{Li-CVPR-Interactiveness} & COCO & \checkmark & ResNet-50 & 17.22 & 13.51 & 18.32 &  & 19.38 & 15.38 & 20.57 \\
no-frills~\cite{Alex-No-Frills} & COCO & \checkmark & ResNet-152 & 17.18 & 12.17 & 18.68 && - & - & -\\
RPNN~\cite{zhou2019relation} & COCO & \checkmark & ResNet-50 & 17.35 & 12.78 & 18.71 & &-&- & - \\
PMFNet~\cite{Bo-PMFNet} & COCO & - & ResNet-50-FPN & 14.92 & 11.42 & 15.96 & & 18.83 & 15.30 & 19.89 \\
PMFNet~\cite{Bo-PMFNet} & COCO & \checkmark & ResNet-50-FPN & 17.46 & \second{15.65} & 18.00 & & \second{20.34} & \second{17.47} & \second{21.20} \\
Peyre~\etal~\cite{peyre2018detecting} & COCO & - & ResNet-50-FPN & \first{19.40} & 14.63 & \first{20.87} & & - & - & - \\
Ours (S-S only)  & COCO & -   & -      & 12.45 & 9.84  & 13.23 & & 15.77 & 12.76 & 16.66 \\
Ours & COCO & - &  ResNet-50-FPN & \second{19.26} & \first{17.74} & \second{19.71} & & \first{23.40} & \first{21.75} & \first{23.89} \\ %app@400K, sp@820K
\midrule
Bansal~\etal~\cite{bansal2019detecting} & HICO-DET & - &  ResNet-101 & \second{21.96} & \second{16.43} & \second{23.62} &  & - & - & - \\
% Ours & HICO-DET & - &  ResNet-50-FPN & 28.62 & 21.30 & 30.80 &  & 31.57 & 24.46 & 33.69 \\
Ours & HICO-DET & - &  ResNet-50-FPN & \first{24.53} & \first{19.47} & \first{26.04} &  & 27.98 & 23.11 & 29.43 \\
% Ours S-S only  & -         & 12.45 & 9.84  & 13.23 & & 15.77 & 12.76 & 16.66 \\
% Ours S-S + App & ResNet-152 & \first{17.54} & \second{14.05} & \second{18.58} & & \first{21.61} & \second{17.82} & \first{22.74} \\ %app@260K, sp@820K
\bottomrule
\end{tabular}

}
\end{table*}


==> [ECCV 2020] HOI arXiv/table/HICO_zeroshot.tex <==
\begin{table}[t]
\centering
\caption{\tb{Zero-shot evaluation on HICO-DET \emph{test} set.} 
}
\label{tab:HICO_zero_shot}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{l cc}
\toprule
\multirow{2}{*}{} &
\multicolumn{2}{c}{Default (Full)}\\
\cline{2-3}
Method  & Unseen (120) & Seen (480)\\
\midrule
Bansal~\etal~\cite{bansal2019detecting} & $11.31\pm1.03$ & $12.74\pm0.34$ \\
Ours   & $16.72\pm1.87$ & $16.84\pm0.58$ \\ 
\bottomrule
\end{tabular}
% }
\end{table}


% H app                                       & 9.31	 & 11.55 & & 13.68 & 15.46 \\ %@340K app
% S-S (one-hot)                                    & 7.89  & 10.26 & & 12.21 & 12.82 \\
% S-S (~\cite{Mikolov-LREC-fastText})             & 9.62  & 12.15 & & 13.43 & 15.27 \\ %@680K sp
% S-S (~\cite{Mikolov-LREC-fastText}) + H app  & 12.27 & 15.86	& & 17.13 & 19.49 \\ %@680K sp + 340K app



% \begin{table}[t]
% \centering
% \caption{\tb{Zero-shot evaluation on HICO-DET \emph{test} set.} 
% }
% \label{tab:HICO_zero_shot}

% \vspace{2mm}
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l cc c  cc}
% \toprule
% \multirow{2}{*}{} &
% \multicolumn{2}{c}{Default (Full)} & &
% \multicolumn{2}{c}{Known Object (Full)}\\
% \cline{2-3} \cline{5-6}
% Method  & Unseen (120) & Seen (480) & & Unseen (120) & Seen (480) \\
% \midrule
% Bansal~\etal~\cite{bansal2019detecting} & $11.31\pm1.03$ & $12.74\pm0.34$ && - & - \\
% % all : $12.45\pm0.16$
% \midrule
% Ours (S-S only)  & $11.85\pm1.54$ & $11.23\pm0.48$ & & $15.01\pm1.77$ & $13.66\pm0.50$ \\ 
% Ours (S-S + H app.)  & $16.72\pm1.87$ & $16.84\pm0.58$ & & $20.58\pm1.93$ & $20.36\pm0.59$ \\ 
% \bottomrule
% \end{tabular}
% % }

==> [ECCV 2020] HOI arXiv/table/VCOCO_ResNet50_results.tex <==
\begin{table}[t]
\centering
\caption{\tb{Results with different feature backbone on the V-COCO $\emph{test}$ set.}
}
\label{tab:VCOCO-ResNet50}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lcccl|c}
\toprule
Method && Use human pose &&  Feature backbone & \textbf{$AP_{role}$} \\
\midrule
Ours   && - && ResNet-50         & 50.7 \\ 
Ours   && - && ResNet-50-FPN     & 51.0 \\ 
\bottomrule
\end{tabular}
% }
\end{table}

==> [ECCV 2020] HOI arXiv/table/VCOCO_ablation.tex <==
\begin{table*}[htbp]
\caption{\textbf{Ablation study on the V-COCO \emph{val} set.} We show the role mAP $AP_{role}$.
}
\label{tab:ablation}

\centering
\mpage{0.5}{
(a) \textbf{More message passing iters.}
} 
\hfill
\mpage{0.45}{
(b) \textbf{Feature used in DRG} 
}
\hfill
\mpage{0.45}{
\begin{tabular}{c|c|c|c}
 iter.    & H graph & O graph & H  + O \\
\hline
 0-iter.  &  48.78 & 47.47 & 50.14 \\
 1-iter.  &  48.83 & 47.35 & 50.74 \\
 2-iter.  &  50.20 & 47.87 & 51.37 \\
\end{tabular}
}
\hfill 
\mpage{0.5}{
\begin{tabular}{l|c}
 & mAP \\
\hline
App. feature (entire image)            & 35.69 \\
App. feature (H-O union box)           & 46.93 \\
Word2vec embedding                           & 37.36 \\
Spatial-semantic feature (ours)              & 51.37 \\
\end{tabular}
}
\hfill 
\\
\mpage{0.35}{
\centering
(c) \textbf{Different subgraph}
} 
\hfill
\mpage{0.6}{
\centering
(d) \textbf{Effectiveness of O subgraph} 
}
\hfill
\mpage{0.35}{
\centering
\begin{tabular}[t]{cc|c}
H graph     & O graph    & mAP   \\
\hline
      -     &      -     & 50.14 \\
 \checkmark &      -     & 51.10 \\
      -     & \checkmark & 50.78 \\
\checkmark & \checkmark  & 51.37 \\
\end{tabular}
}
\hfill
\mpage{0.6}{
\centering
\begin{tabular}[t]{l|cccc}
                             & 1-3 & 4-6 & 7+ & all  \\
\hline
H graph                      & 57.89 & 52.77 & 50.96 & 51.10 \\
H graph + O graph            & 58.28 & 53.75 & 51.06 & 51.37 \\
Margin                       & +0.39 & +0.98 & +0.10 & +0.27 \\
\% of testing images         & 68\%  & 12\%  & 20\%  & 100\% \\
\end{tabular}
}
\end{table*}

\vspace{-2.0mm}









% \begin{table$\times$}[t]
% \centering
% \caption{\textbf{Deeper feature refinement modules:} we compare 0, 1, 2, 3, and 4 feature refinement modules added to the baseline. Ablation is conducted on the V-COCO \texttt{val} set.}
% \label{tab:ablation_numFRM}
% \vspace{2mm}
% \begin{tabular}{c|cc}
% \toprule
%    model     & \multicolumn{2}{c}{$AP_{role}$ } \\
%              & sp w/ feature refinement & sp w/ feature refinement + appearance \\
% \midrule
%  0-block  & 38.9 & 45.1 \\
%  1-block  & 41.1 & 46.3 \\
%  2-block  & 43.1 & 47.4 \\
%  3-block  & 43.6 & 47.5 \\
%  4-block  & 43.9 & 47.9 \\
% \bottomrule
% \end{tabular}
% \end{table$\times$}

% % \begin{table$\times$}[t]
% % \centering
% % \caption{\textbf{Spatial representation:} we compare different spatial representations}
% % \label{tab:ablation_sp}

% % \vspace{2mm}
% % \begin{tabular}{l|cc}
% % \toprule
% %  spatial representation     & \multicolumn{2}{c}{$AP_{role}$ } \\
% %              & sp w/ feature refinement & sp w/ feature refinement + appearance \\
% % \midrule
% %  2 channel pattern  & 43.1 & 47.4 \\
% %  10-dim vector      & -  & - \\
% % \bottomrule
% % \end{tabular}
% % \end{table$\times$}

% \begin{table$\times$}[t]
% \centering
% \caption{\textbf{Word embedding:} we compare different word embeddings}
% \label{tab:ablation_word}

% \vspace{2mm}
% \begin{tabular}{l|cc}
% \toprule
%  word embedding     & \multicolumn{2}{c}{$AP_{role}$ } \\
%              & sp w/ feature refinement & sp w/ feature refinement + appearance \\
% \midrule
%  fastText  &  43.1 & 47.4 \\
%  one-hot vector  & 39.5 & 46.0 \\
% \bottomrule
% \end{tabular}
% \end{table$\times$}

% \begin{table$\times$}[t]
% \centering
% \caption{\textbf{Statistics prior:} we explore the contribution of using statistics prior}
% \label{tab:ablation_prior}

% \vspace{2mm}
% \begin{tabular}{c|c}
% \toprule
%  statistics prior     & $AP_{role}$ \\
% \midrule
%  -  &  47.4 \\
% \checkmark  & \tb{48.5} \\
% soft  & 47.2 \\
% \bottomrule
% \end{tabular}
% \end{table$\times$}

% \begin{table$\times$}[t]
% \centering
% \caption{\textbf{Fusion options:} we explore different ways to fuse the prediction}
% \label{tab:ablation_fusion}

% \vspace{2mm}
% \begin{tabular}{c|c}
% \toprule
% fusion & $AP_{role}$ \\
%        & sp w/ feature refinement + appearance \\
% \midrule
%  H + O + sp    & 45.1 \\
%  H $\times$ O $\times$ sp    & 46.4 \\
% (H + O) $\times$ sp   & 47.4 \\
% fusion by MLP  &  -   \\
% \bottomrule
% \end{tabular}
% \end{table$\times$}



% \begin{table$\times$}[t]
% \centering
% \caption{\textbf{Contribution of appearance and feature refinement module}}
% \label{tab:ablation_compare}

% \vspace{2mm}
% \begin{tabular}{l|cc}
% \toprule
%  appearance     & \multicolumn{2}{c}{$AP_{role}$ } \\
%  & sp  & sp w/ feature refinement \\
% \midrule
% $\emptyset$    & 38.9 & 43.1 \\
% H              & 40.7 & 44.9 \\
% H + O          & 45.1 & 47.4 \\
% H + O w/ iCAN  & 45.7 & 47.5 \\
% \bottomrule
% \end{tabular}
% \end{table$\times$}



%% ECCV before camera ready
% \begin{table*}[htbp]
% \caption{\textbf{Ablation study on the V-COCO \emph{val} set.} We show the role mAP $AP_{role}$.
% }
% \label{tab:ablation}

% % \vspace{0.5mm}
% %
% \centering
% (a) \textbf{More message passing iterations} 
% % Deeper network has better performance.
% \\
% % \mpage{0.45}{
% \centering
% \begin{tabular}{c|c|c|c}
% iter. & H subgraph  & O subgraph & H subgraph + O subgraph\\
% \hline
% %  0-iter.  & 57.68 & 55.69 & 58.21 \\
% %  1-iter.  & 58.00 & 56.28 & 58.56 \\
% %  2-iter.  & 58.85 & 56.76 & 59.44 \\
%  0-iter.  & 48.78 & 47.47 & 50.14 \\
%  1-iter.  &  48.83 & 47.35 & 50.74 \\
%  2-iter.  &  50.20 & 47.87 & 51.37 \\
% \end{tabular}
% \hfill 
% \\
% \vspace{4mm}
% \begin{minipage}{0.45\linewidth}
% {(b) \textbf{Different subgraph}
% } 
% \end{minipage}
% \hfill
% \begin{minipage}{0.45\linewidth}
% {(c) \textbf{Score fusion options} 
% % Performance when using different score fusion methods.
% }
% \end{minipage}
% \hfill
% % \vspace{3mm}
% \hfill
% \mpage{0.45}{
% % \centering
% % \vspace{-4mm}
% \begin{tabular}[t]{cc|c}
% H subgraph & O subgraph & mAP   \\
% \hline
% % % sph_0ssar*spo_0ssar*h*o
% %       -     &      -     &  58.21 \\
% % % sph_2ssar*spo_0ssar*h*o
% %  \checkmark &      -     &  58.84 \\
% % % sph_0ssar*spo_2ssar*h*o 
% %       -     & \checkmark &  59.23 \\
% % % sph_2ssar*spo_2ssar*h*o
% % \checkmark & \checkmark  &  59.44 \\
% % sph_0ssar*spo_0ssar*h*o
%       -     &      -     & 50.14 \\
% % sph_2ssar*spo_0ssar*h*o
%  \checkmark &      -     & 51.10 \\
% % sph_0ssar*spo_2ssar*h*o 
%       -     & \checkmark & 50.78 \\
% % sph_2ssar*spo_2ssar*h*o
% \checkmark & \checkmark  & 51.37 \\
% \end{tabular}
% }
% \hfill
% \mpage{0.45}{
% \centering
% \begin{tabular}{c|c}
% Fusion & mAP \\
% % \midrule
% \hline
% % ($s^a_{h}$ + $s^a_{o}$) + ($s^a_{spH}$ + $s^a_{spO}$)                      & 58.25 \\
% % ($s^a_{h}$ $\cdot$ $s^a_{o}$) $\cdot$ ($s^a_{spH}$ + $s^a_{spO}$)        & 58.77 \\
% % ($s^a_{h}$ + $s^a_{o}$) $\cdot$ ($s^a_{spH}$ + $s^a_{spO}$)               & 59.11 \\
% % ($s^a_{h}$ + $s^a_{o}$) $\cdot$ ($s^a_{spH}$ $\cdot$ $s^a_{spO}$)        & 59.19 \\
% % ($s^a_{h}$ $\cdot$ $s^a_{o}$) $\cdot$ ($s^a_{spH}$ $\cdot$ $s^a_{spO}$) & 59.44 \\

% ($s^a_{h}$ $\times$ $s^a_{o}$) $\times$ ($s^a_{spH}$ + $s^a_{spO}$)        & 50.05 \\
% ($s^a_{h}$ + $s^a_{o}$) + ($s^a_{spH}$ + $s^a_{spO}$)                      & 50.57 \\
% ($s^a_{h}$ + $s^a_{o}$) $\times$ ($s^a_{spH}$ + $s^a_{spO}$)               & 51.09 \\
% ($s^a_{h}$ + $s^a_{o}$) $\times$ ($s^a_{spH}$ $\times$ $s^a_{spO}$)        & 51.35 \\
% ($s^a_{h}$ $\times$ $s^a_{o}$) $\times$ ($s^a_{spH}$ $\times$ $s^a_{spO}$) & 51.37 \\
% \end{tabular}
% }
% \hfill
% \vspace{\tabmargin}
% \end{table*}


==> [ECCV 2020] HOI arXiv/table/VCOCO_mAP.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Detailed results on V-COCO \emph{test} set.} The best performance is in \first{bold} and the second best is \second{underscored}.} 
% \jiarui{the score of interactiveness in github is higher than what they show in their paper. They report 48.96 in github, while in paper it is 48.7.} 
% \resizebox{0.8\columnwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
& {InteractNet~\cite{Gkioxari-CVPR-InteractNet} } & {iCAN~\cite{Gao-BMVC-iCAN}} & ${RP_{T2}C_D}^\star$~\cite{Li-CVPR-Interactiveness} & {Ours} \\
& ResNet-50-FPN & ResNet-50 & ResNet-50 & ResNet-50-FPN \\
\midrule
carry 			 & 33.1 & 32.0 & \second{40.8} &\first{41.3} \\
catch 			 & 42.5 & 47.6 & \second{48.4} &\first{49.3} \\
drink			 & 33.8 & 32.2 & \second{34.4} &\first{35.5} \\
hold 		     & 26.4 & 29.1 & \second{37.3} & \first{40.7} \\
jump  		     & 45.1 & 51.5 & \second{53.8} & \first{54.2} \\
kick  			 & \second{69.4} & 66.9 & 66.3 & \first{69.8} \\
lay   			 & 21.0 & 22.4 & \first{29.6} & \second{26.1} \\
look 			 & 20.2 & 26.5 & \second{32.3} & \first{35.5} \\
read     		 & 23.9 & \second{30.7} & 29.9 & \first{39.5} \\
ride             & 55.2 & 61.9 & \second{66.3} & \first{69.9} \\
sit              & 19.9 & 26.0 & \first{31.6} & \second{31.4} \\
skateboard       & 75.5 & 79.4 & \second{83.4} & \first{85.9} \\
ski              & 36.5 & 41.7 & \second{50.0} & \first{52.9} \\
snowboard        & 63.9 & \second{74.4} & 71.6 & \first{75.6} \\
surf             & 65.7 & 77.2 & \second{79.7} & \first{80.6} \\
talk-on-phone    & 31.8 & 52.8 & \second{53.6} & \first{55.9} \\
throw            & 40.4 & 40.6 & \second{43.3} & \first{52.1} \\
work-on-computer & 57.3 & 56.3 & \first{65.5} & \second{64.3} \\
\midrule
\multirow{2}{*}{cut} \ \ (object) & 23.0 & 34.8 & \second{40.1} & \first{42.4} \\
\qquad (instrument) & 36.4 & 37.2 & \first{41.6} & \second{39.9} \\
\multirow{2}{*}{eat} \ \ (object) & 32.4 & 37.7 & \second{39.1} & \first{41.9} \\
\qquad (instrument) & 2.0  & \second{8.3}  & \first{9.4} & 5.9  \\
\multirow{2}{*}{hit} \ \ (object) & \first{62.3} & 46.1 & 52.6 & \second{54.7} \\
\qquad (instrument) & 43.3 & 74.1 & \second{74.4} & \first{77.6} \\
\midrule
\textbf{mean AP role} & 40.0 & 45.3 & \second{49.0} & \first{51.0} \\
\bottomrule
\end{tabular}
% }
\label{tab:VCOCO}
\end{table}


==> [ECCV 2020] HOI arXiv/table/VCOCO_more_ablation.tex <==
\begin{table*}[htbp]
\caption{\textbf{More Ablation study on the V-COCO \emph{val} set.} We show the $AP_{role}$. % \chen{Title looks weird.}
%\jiabin{
%(b) Show the actual number of parameters in the SSAR stream. 
%(c)
%}
}
\label{tab:more_ablation}
%
\begin{minipage}{0.5\linewidth}
{(a) \textbf{Shared SSAR modules:} Stacking more shared modules improves the performance without increasing the model size.}
\end{minipage}
%
\hfill
%
\begin{minipage}{0.45\linewidth}
{(b) \textbf{Category representation}: All of the category representation approaches achieve good performance.} 
\end{minipage}
\\
\mpage{0.45}{
\centering
\begin{tabular}{c|cc|cc}
      & \multicolumn{2}{c}{Separate} & \multicolumn{2}{c}{Shared} \\
model & S-S only & S-S + App. & S-S only & S-S + App. \\
\midrule
 1-block  & 41.1 & 46.3 & 41.1 & 46.3 \\
 \midrule
 2-block  & 43.1 & 47.4 & 43.0 & 47.3 \\
 3-block  & 43.6 & 47.5 & 43.9 & 48.1 \\
 4-block  & 43.9 & 47.9 & 44.2 & 48.1 
\end{tabular}
}
\hfill
\mpage{0.45}{ \centering
\begin{tabular}{l|cc}
 Category representation  & S-S only & S-S + App. \\
\midrule
 $\emptyset$ (no object category info.) & 13.1 & 38.8 \\
 one-hot vector                         & 39.5 & 46.0 \\
 word2vec~\cite{Mikolov-NIPS-Word2vec}  & 44.3 & 48.2 \\
 GloVe~\cite{Pennington-EMNLP-Glove}    & 44.4 & 48.1 \\
 fastText~\cite{Mikolov-LREC-fastText}  & 43.1 & 47.4 
\end{tabular}
}
\hfill
\end{table*}



==> [ECCV 2020] HOI arXiv/table/VCOCO_results.tex <==
\begin{table}[t]
\centering
\caption{\tb{Comparison with the state-of-the-art on the V-COCO $\emph{test}$ set.} The best performance is in \first{bold} and the second best is \second{underscored}. Character $^\star$ indicates that the method uses both VCOCO and HICO-DET training data.
%
``S-S only'' shows the performance of our spatial-semantic stream.
}
\label{tab:vcoco_comparison}
% \resizebox{0.6\linewidth}{!}
{
\begin{tabular}{lccl|c}
\toprule
Method & Use human pose &&  Feature backbone & \textbf{$AP_{role}$} \\
\midrule
VSRL~\cite{Gupta-SemanticRoleLabeling}              & - && ResNet-50-FPN    & 31.8 \\
InteractNet~\cite{Gkioxari-CVPR-InteractNet}        & - && ResNet-50-FPN    & 40.0 \\
BAR-CNN~\cite{Kolesnikov-BAR}                       & - && Inception-ResNet & 41.1 \\
GPNN~\cite{Qi-ECCV-GraphParsing}                    & - && ResNet-101       & 44.0 \\
iCAN~\cite{Gao-BMVC-iCAN}                           & - && ResNet-50        & 45.3 \\
Wang et al. ~\cite{wang2019deep} & - && ResNet-50 & 47.3 \\
RPNN~\cite{zhou2019relation} & \checkmark && ResNet-50 & 47.5 \\
% $RP_DC_D$~\cite{Li-CVPR-Interactiveness}            & ResNet-50  & 47.8 \\
${RP_{T2}C_D}^\star$~\cite{Li-CVPR-Interactiveness} & \checkmark && ResNet-50        & 48.7 \\
PMFNet \cite{Bo-PMFNet}                             & - && ResNet-50-FPN    & 48.6 \\
PMFNet \cite{Bo-PMFNet}                             & \checkmark && ResNet-50-FPN    & \first{52.0} \\
% \midrule
% Ours Human S-S only                     & $\times$ & & -           & 46.62 \\
% Ours Object S-S only                     & $\times$ & & -           & 42.28 \\
Ours (S-S only)                               & - & & -           & 47.1 \\
Ours                                                & - && ResNet-50-FPN    & \second{51.0} \\
\bottomrule
\end{tabular}
}
\end{table}

==> [ECCV 2020] HOI arXiv/table/obj_representation.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Object category representation.} Representing object category using word embedding works best.} 
%  \resizebox{\columnwidth}{!}{
\begin{tabular}{l|cc}
 Category representation  & S-S only & S-S + App. \\
\midrule
 $\emptyset$ (no object category info.) & 13.1 & 38.8 \\
 O app.                                 & 42.8 & 45.9 \\
 one-hot vector                         & 43.2 & 47.0 \\
 fastText~\cite{Mikolov-LREC-fastText}  & \textbf{44.3} & \textbf{47.2}
\end{tabular}
\label{tab:obj_representation}
\end{table}


==> [ECCV 2020] HOI arXiv/table/word_dim.tex <==
\begin{table}[t]
\caption{\textbf{Different dimensions of the word embedding.} Performance when using different dimensions of the word embedding. We show the role mAP $AP_{role}$ on V-COCO \emph{val} set.}
\label{tab:word_dim}

\mpage{0.45}{ \centering
\begin{tabular}{l|c}
Word dim.  & S-S only \\
\midrule
10  & 45.85 \\
20  & 45.96 \\
40  & 45.99 \\
80  & 46.09 \\
160 & 46.16 \\
300 & 46.00 \\
\end{tabular}
}
\hfill
\begin{minipage}{0.45\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/dim.pdf}}
\end{minipage}
\end{table}

==> figure/fig_HCVRD_more.tex <==
\begin{figure*}[t]
\centering

% HCVRD
\mfigure{0.151}{{figure_HCVRD/holds_420_37.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_910_249.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_2333_57.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_3453_4.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_3453_479.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/holds_713118_274.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HCVRD/in_87_494.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_323_499.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_408_369.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_455_273.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_1615_451.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/in_4587_130.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HCVRD/wearing_3185_156.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_3235_280.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_3548_261.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_4587_180.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_4611_481.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/wearing_4982_235.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HCVRD/with_355_513.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_420_37.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_637_302.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_2383_149.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_2870_1.jpg}}\hfill
\mfigure{0.151}{{figure_HCVRD/with_713352_22.jpg}}\\
% \vspace{0.5mm}
% \vspace{\figcapmargin}
% \captionof{figure}{\textbf{HOI detection results on the HCVRD \emph{test} set.}}
\caption{\textbf{HOI detection results on HCVRD \emph{test} set.}}
\label{fig:HCVRD_more}
\end{figure*}

==> figure/fig_HICO_more.tex <==
\begin{figure*}[t]
\centering

% HICO
\mfigure{0.151}{{figure_HICO/carry_000000003392_218.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000003535_115.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000006088_103.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000006501_3.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000008037_101.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/carry_000000008849_414.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/wear_000000000874_52.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000000906_128.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000001045_122.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000001980_253.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000003565_281.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/wear_000000009605_23.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/board_000000000018_442.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/ride_000000001551_241.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000002640_94.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000004704_211.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000006379_284.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/board_000000008525_394.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/eat_000000002327_208.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000004013_200.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000006943_175.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000008015_54.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000008635_104.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/eat_000000008983_17.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/feed_000000003253_111.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000006182_327.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000006463_4.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000007259_0.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000008156_386.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/feed_000000008575_2.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/hold_000000000073_125.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000248_250.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000275_130.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000277_19.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000412_99.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/hold_000000000523_2.jpg}}\\
% \vspace{0.5mm}
\mfigure{0.151}{{figure_HICO/read_000000000412_99.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000002774_354.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000005884_101.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000006963_83.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000007579_245.jpg}}\hfill
\mfigure{0.151}{{figure_HICO/read_000000007871_1.jpg}}\\
% \vspace{0.5mm}
% \vspace{\figcapmargin}
% \captionof{figure}{\textbf{More HOI detection results on the HICO-DET \emph{test} set.}}
\caption{\textbf{HOI detection results on HICO-DET \emph{test} set.}}
\label{fig:HICO_more}
\end{figure*}

==> figure/fig_HICO_not_annotated.tex <==
\begin{figure*}[t]
\centering
\newlength\ftsa
\setlength\ftsa{3cm} % page-width size
\newlength\ftsb
\setlength\ftsb{0.0mm}
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002714_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/ride_000000001454_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002464_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/straddle_000000000011_gt.jpg}\vspace{\ftsb}\\%
 Ground truth}%
%
\hfill%
%
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002714_3.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/ride_000000001454_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002464_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/straddle_000000000011_1.jpg}\vspace{\ftsb}\\%
 Our detections}%
%
\hfill%
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002506_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/read_000000000874_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000001297_gt.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/hold_000000001529_gt.jpg}\vspace{\ftsb}\\%
 Ground truth}%
%
\hfill%
\parbox[t]{\ftsa}{\vspace{0mm}\centering%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000002506_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/read_000000000874_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/sit_on_000000001297_1.jpg}\vspace{\ftsb}\\%
\includegraphics[width=\ftsa]{figure_HICO_not_annotated/hold_000000001529_1.jpg}\vspace{\ftsb}\\%
 Our detections}%
\vspace{\figcapmargin}
\caption{\textbf{HICO-DET is not fully annotated.}
The first and third column shows \emph{all} the ground truth annotations. The second and last column shows the HOI detection from our model. While our method correctly detects the HOIs, we are penalized because the dataset is not fully annotated.
}
\label{fig:HICO_not_annotated}
\end{figure*}


% \begin{figure*}[t]
% \centering
% \newlength\ftsa
% \setlength\ftsa{3cm} % page-width size
% \newlength\ftsb
% \setlength\ftsb{0.0mm}
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_sp.png}\vspace{\ftsb}\\%
% \scriptsize Spatial only}%
% %
% \hfill%
% %
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_O.png}\vspace{\ftsb}\\%
% \scriptsize Spatial+ Obj App.}%
% %
% \hfill%
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_onehot.png}\vspace{\ftsb}\\%
% \scriptsize Spatial + One-hot vec.}%
% %
% \hfill%
% \parbox[t]{\ftsa}{\vspace{0mm}\centering%
% \includegraphics[width=\ftsa]{figure_tsne/Tsne_fastText_0.png}\vspace{\ftsb}\\%
% \scriptsize Spatial + fastText}%
% \caption{\textbf{t-SNE visualization of different object category representation.}
% }
% \label{fig:tsne}
% \end{figure*}



==> figure/fig_Tsne.tex <==
\begin{figure*}[t]
\centering
% \newlength\ftsa
\setlength\ftsa{3cm} % page-width size
% \newlength\ftsb
\setlength\ftsb{0.0mm}
\parbox[t]{\ftsa}{
\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_sp.png}\\%
\scriptsize Spatial only}%
%
\hfill%
%
\parbox[t]{\ftsa}{\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_O.png}\\%
\scriptsize Spatial+ Obj App.}%
%
\hfill%
\parbox[t]{\ftsa}{\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_onehot.png}\\%
\scriptsize Spatial + One-hot vec.}%
%
\hfill%
\parbox[t]{\ftsa}{\centering%
\includegraphics[width=\ftsa]{figure_tsne/Tsne_fastText_0.png}\\%
\scriptsize Spatial + fastText}%
\caption{\textbf{t-SNE visualization of different object category representation.}
}
\label{fig:tsne}
\end{figure*}



==> figure/fig_Tsne_DRG.tex <==
\begin{figure*}[t]
\centering

\newlength\ffca
\setlength\ffca{4cm} % page-width size
\newlength\ffcb
\setlength\ffcb{-0.0mm}

\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/Tsne_fastText_0.png}\\%
 Human-centric 0 iter.}%
%
\hfill%
%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/Tsne_fastText_1.png}\\%
 Human-centric 1 iter.}%
%
\hfill%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/Tsne_fastText_2.png}\\%
 Human-centric 2 iter.}%
%
\hfill%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/tsne_object_centric_0.png}\\%
 Object-centric 0 iter.}%
%
\hfill%
%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/tsne_object_centric_1.png}\\%
 Object-centric 1 iter.}%
%
\hfill%
\parbox[t]{\ffca}{\centering%
\includegraphics[width=\ffca]{figure_tsne/tsne_object_centric_2.png}\\%
 Object-centric 2 iter.}%
\mfigure{0.7}{{fig/color_bar.png}}\\
\vspace{2mm}
\caption{\textbf{t-SNE visualization of spatial-semantic representation with different iterations of feature aggregation.}
}
\label{fig:tsne_DRG}
\end{figure*}

==> figure/fig_VCOCO_more.tex <==
\begin{figure*}[t]
\centering

% V-COCO
\mfigure{0.151}{{figure_VCOCO/carry_000000301867_251.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000550714_0.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000144863_0.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000543570_199.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hold_000000012991_50.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hold_000000427615_170.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/ski_000000010142_320.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/snowboard_000000149014_198.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000062363_367.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/talk_000000263351_5.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/skateboard_000000541017_43.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/jump_000000186721_351.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/catch_000000015846_197.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/cut_000000091318_4.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000121442_282.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000003716_218.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hold_000000032334_96.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/kick_000000282225_328.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/hold_000000256983_141.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000310035_341.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000032300_167.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000186711_298.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/work_000000086011_44.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000087740_119.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/look_000000153717_329.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000276024_237.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000504353_84.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/throw_000000404517_57.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000413044_113.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/kick_000000204137_280.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/sit_000000223414_216.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/carry_000000247264_422.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/cut_000000012991_50.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/skateboard_000000412975_1.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000437540_375.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/throw_000000072376_264.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/cut_000000314074_0.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000358231_267.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000180764_2.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/sit_000000526904_91.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000432623_350.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000137297_134.jpg}} 
\\

\mfigure{0.151}{{figure_VCOCO/hit_000000306335_265.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/snowboard_000000001700_212.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000032300_305.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/lay_000000276893_202.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000106617_1.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000509471_178.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/work_000000526904_91.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/look_000000543570_253.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ski_000000341719_320.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000567494_247.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/eat_000000204432_122.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/sit_000000577614_400.jpg}}
\\

\mfigure{0.151}{{figure_VCOCO/talk_000000528729_169.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/surf_000000295316_189.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/snowboard_000000564743_227.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ski_000000346589_90.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/hit_000000485673_125.jpg}}\hfill
\mfigure{0.151}{{figure_VCOCO/ride_000000480408_117.jpg}}
\\
\caption{\textbf{HOI detection results on V-COCO \emph{test} set.}}
\label{fig:VCOCO_more}
\end{figure*}

==> figure/fig_error.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}{0.45\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/iCAN_error.pdf}}
\end{minipage}
%
\hfill
\begin{minipage}{0.45\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/DRG_error.pdf}}
\end{minipage}
\hfill
\begin{minipage}{0.07\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/Legend.pdf}}
\end{minipage}
\\
\mpage{0.48}{(a) iCAN} \hfill
\mpage{0.48}{(b) DRG} \hfill
\\
\captionof{figure}{
\textbf{Comparison of the distribution of the error categories between iCAN and our proposed DRG.} We show the distribution of the incorrect detections for each action class. \tb{`incorrect label'} refers to the detected person is predicted to perform an action which he does not. \tb{`bck'} indicates the object detector fails to localize the person (IoU with any ground truth person is less than 0.1). \tb{`person misloc'} means the detected person is not localized well (IoU is between $0.1$ and $0.5$ with a ground truth person) regardless of the related object. \tb{`object misloc'} refers to the detected object is not localized well while the related person is successfully localized. \tb{`mis-grouping'} indicates the person is successfully localized, but the network fails to match the person to the correct related object (IoU between the ground truth associated object and the predicted object is less than 0.1). \tb{`occlusion'} means we incorrectly associate an object with a correct detected person, while the object is not annotated in the ground truth due to occlusions.
%
\tb{Discussion:} our proposed DRG helps most with the mis-grouping. By leveraging the proposed human-centric subgraph and object-centric subgraph, we can enhance the correct HOIs and suppress the unrelated pairs. As a result, the mis-grouping error is reduced, especially for the action classes that humans and objects have a typical spatial relationship, \eg $\textit{hit obj}$, $\textit{hit instr}$, and $\textit{skateboard instr}$.
}
\label{fig:error}
\end{figure*}

==> figure/fig_failure_more.tex <==
\begin{figure*}[t]
\centering
\mfigure{0.155}{{figure_failure/incorrect_obg_look_000000072376_264.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_obj_hit_000000375021_160.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_ride_000000424464_48.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_ride_000000171548_307.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_work_000000149783_220.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_eat_000000023807_233.jpg}}\hfill
\\
\mfigure{0.155}{{figure_failure/incorrect_obj_sit_000000472256_206.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_obj_eat_000000041279_45.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_skateboard_000000002179_220.jpg}}\hfill
\mfigure{0.155}{{figure_failure/incorrect_action_sit_000000032334_96.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_sit_000000025603_338.jpg}}\hfill
\mfigure{0.155}{{figure_failure/mis_group_ride_000000370657_404.jpg}}\hfill
\\

\mpage{0.31}{Incorrect object} \hfill
\mpage{0.31}{Incorrect action} \hfill
\mpage{0.31}{Mis-grouping}
\caption{
%
\textbf{More failure cases.} 
}
\label{fig:failure_more}
\end{figure*}

==> figure/fig_module.tex <==
\begin{figure*}[t]
\includegraphics[width=\linewidth]{fig/SSAR.pdf}
\caption{
%
\textbf{SSAR module.} To recognize the interaction between the $i$-th person and the $j$-th object, we first pair the $i$-th person with all $N$ objects in an image. Given the spatial relation between the $i$-th person and the $j$-th object, as well as the word embedding of the $j$-th object's category, we generate a spatial-semantic representation $\mathbf{x}_{i,j}$ by concatenating the convolved $64 \times 64 \times 2$ spatial pattern with the $300D$ word embedding vector.
%
We aggregate all the spatial-semantic features which involved the same person, \ie $\{\mathbf{x}_{i, j^\prime}| j^\prime \in \{1 \cdots N\}\}$, to obtain the aggregated spatial-semantic features $\mathbf{x}_{i, j}^{\prime\prime}$.
%
\ignorethis{
We use the linear transformation $W_Q$ and $W_K$ to generate the query $\mathbf{q}_{i, j}$ and key $\mathbf{k}_{i, j^\prime}$. 
%
We obtain the attention weights by performing the scaled dot-product attention of the query over the key features. 
%
The spatial-semantic representation $\mathbf{x}_{i, j}^\prime$ is an attentioal weighted sum of all spatial-semantic representations of this person, transformed by $W_V$.
%
We apply a dropout to $\mathbf{x}_{i, j}^\prime$ and add it to the original feature $\mathbf{x}_{i, j}$.
%
We finally pass $\mathbf{x}_{i, j}^\prime$ through LayerNorm and yield the aggregated feature $\mathbf{x}_{i, j}^{\prime\prime}$. 
}
%
% We use $\mathbf{x}_{i, j}^{(0)}$ to denote the initial spatial-semantic feature. We use $\mathbf{x}_{i, j}^{(k)}$ to denote the aggregated feature after $k$ SSAR module.
}
\label{fig:module}
\end{figure*}

==> figure/fig_multi_action.tex <==
\begin{figure}[t]
\centering
\mfigure{0.32}{figure_multi_action/eat_000000146120_273_1.jpg}\hfill
\mfigure{0.32}{figure_multi_action/hold_000000146120_273_3.jpg}\hfill
\mfigure{0.32}{figure_multi_action/sit_000000146120_273_2.jpg}
% \\
% \mfigure{0.32}{figure_multi_action/eat_000000132272_173_1.jpg}\hfill
% \mfigure{0.32}{figure_multi_action/hold_000000132272_173_3.jpg}\hfill
% \mfigure{0.32}{figure_multi_action/drink_000000132272_173_2.jpg}
\\
\caption{
\textbf{Detecting multiple actions.} Our model can detect a person doing different actions with different objects.
}
\label{fig:multi_action}
\end{figure}

==> figure/fig_multi_action_more.tex <==
\begin{figure*}[t]
\centering
\mfigure{0.152}{{figure_multi_action/hold_000000007298_183_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/catch_000000007298_183_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000007298_183_3.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/sit_000000577614_400_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000577614_400_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/work_000000577614_400_3.jpg}}\hfill
\\
\mfigure{0.152}{{figure_multi_action/hold_000000567494_247_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/hit_000000567494_247_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000567494_247_3.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/sit_000000300330_70_1.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/look_000000300330_70_2.jpg}}\hfill
\mfigure{0.152}{{figure_multi_action/work_000000300330_70_3.jpg}}\hfill
\\
\caption{
\textbf{Detecting multiple actions.} Our model can detect a person doing different actions with different objects. 
}
\label{fig:multi_action_more}
\end{figure*}

==> table/HCVRD_results.tex <==
\begin{table}[t]
\centering
\caption{\tb{Performance comparison with the state-of-the-art on the HCVRD $\emph{test}$ set.} The performance is measured by Recall@50 (R@50) and Recall@100  (R@100) under two different settings, namely top-1 and top-3. The best performance is in \first{bold} and the second best is \second{underscored}. Character $^\star$ indicates that the results are reported by \cite{wang2019deep}.
}
\label{tab:HCVRD_comparison}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lc|cc|cc}
\toprule
       &                  & \multicolumn{4}{c}{Predicate Det.} \\
Method & Feature backbone & \multicolumn{2}{c}{R@50} & \multicolumn{2}{c}{R@100} \\
       &                  & top-1 & top-3 & top-1 & top-3 \\
\midrule
Multilabel~\cite{Zhuang-AAAI-HCVRD}         & VGG-16     & 0.9  & 2.8  & 0.9  & 2.8  \\
JointCNN~\cite{Zhuang-AAAI-HCVRD}           & VGG-16     & 2.7  & 7.4  & 2.7  & 7.4  \\
SeparateCNN~\cite{Zhuang-AAAI-HCVRD}        & VGG-16     & 29.0 & 44.4 & 29.0 & 45.9 \\
Webly-Supervised~\cite{Zhuang-AAAI-HCVRD}   & VGG-16     & 31.1 & 47.7 & 31.1 & 49.0 \\
iCAN$^\star$~\cite{Gao-BMVC-iCAN} & ResNet-50 & 33.8 &  48.9 & 33.8 & 49.4 \\
Wang et al. ~\cite{wang2019deep}            & ResNet-50  & 37.1 & 51.3 & 37.1 & 51.9 \\
% \midrule
Ours (S-S only)                             & -          & \second{38.1} & \second{61.8} & \second{38.1} & \second{62.2} \\
% Ours                                        & VGG-16 & - & - & - & - \\
Ours                                        & ResNet-50-FPN & \first{43.6} & \first{65.5} & \first{43.6} & \first{65.9} \\
\bottomrule
\end{tabular}
% }
\end{table}


% Multilabel~\cite{Zhuang-AAAI-HCVRD}         & VGG-16     & 0.9  & 2.8  & 0.9  & 2.8  \\
% JointCNN~\cite{Zhuang-AAAI-HCVRD}           & VGG-16     & 2.7  & 7.4  & 2.7  & 7.4  \\
% SeparateCNN~\cite{Zhuang-AAAI-HCVRD}        & VGG-16     & 29.0 & 44.4 & 29.0 & 45.9 \\
% Webly-Supervised~\cite{Zhuang-AAAI-HCVRD}   & VGG-16     & 31.1 & 47.7 & 31.1 & 49.0 \\
% \midrule
% Ours (S-S only)                              & -             & \textbf{46.4} & \underline{65.3} & \textbf{46.4} & \underline{65.8} \\
% Ours                             & ResNet-50-FPN  & \textbf{46.4} & \textbf{65.6} & \textbf{46.4} & \textbf{66.0} \\

==> table/HICO_Resnet50_results.tex <==
\begin{table*}[t]
\centering
\caption{\tb{Results with different feature backbone on the HICO-DET $\emph{test}$ set.}
For the object detector, ``COCO'' means that the detector is trained on COCO, while ``HICO-DET'' means that the detector is first pre-trained on COCO and then further fine-tuned on HICO-DET.
}
\label{tab:HICO_Resnet50}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l cc l ccc c  ccc}
\toprule
\multirow{4}{*}{} & &&&
\multicolumn{3}{c}{Default} & &
\multicolumn{3}{c}{Known Object}\\
\cline{5-7} \cline{9-11}
Method & Detector & Use human pose & Feature backbone & Full & Rare & Non Rare &  & Full & Rare & Non Rare  \\
\midrule
Ours  & COCO & -   & ResNet-50     & 18.87 & 16.90  & 19.45 & & 22.83 & 20.61 & 23.49 \\
Ours & COCO & - &  ResNet-50-FPN & 19.26 & 17.74 & 19.71 & & 23.40 & 21.75 & 23.89 \\ 
\midrule
Ours & HICO-DET & - &  ResNet-50 & 24.05 & 18.72 & 25.65 &  & 27.39 & 22.01 & 28.99 \\
Ours & HICO-DET & - &  ResNet-50-FPN & 24.53 & 19.47 & 26.04 &  & 27.98 & 23.11 & 29.43 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> table/HICO_zeroshot.tex <==
\begin{table}[t]
\centering
\caption{\tb{Zero-shot evaluation on HICO-DET \emph{test} set.} 
}
\label{tab:HICO_zero_shot}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{l cc}
\toprule
\multirow{2}{*}{} &
\multicolumn{2}{c}{Default (Full)}\\
\cline{2-3}
Method  & Unseen (120) & Seen (480)\\
\midrule
Bansal~\etal~\cite{bansal2019detecting} & $11.31\pm1.03$ & $12.74\pm0.34$ \\
Ours   & $16.72\pm1.87$ & $16.84\pm0.58$ \\ 
\bottomrule
\end{tabular}
% }
\end{table}


% H app                                       & 9.31	 & 11.55 & & 13.68 & 15.46 \\ %@340K app
% S-S (one-hot)                                    & 7.89  & 10.26 & & 12.21 & 12.82 \\
% S-S (~\cite{Mikolov-LREC-fastText})             & 9.62  & 12.15 & & 13.43 & 15.27 \\ %@680K sp
% S-S (~\cite{Mikolov-LREC-fastText}) + H app  & 12.27 & 15.86	& & 17.13 & 19.49 \\ %@680K sp + 340K app



% \begin{table}[t]
% \centering
% \caption{\tb{Zero-shot evaluation on HICO-DET \emph{test} set.} 
% }
% \label{tab:HICO_zero_shot}

% \vspace{2mm}
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l cc c  cc}
% \toprule
% \multirow{2}{*}{} &
% \multicolumn{2}{c}{Default (Full)} & &
% \multicolumn{2}{c}{Known Object (Full)}\\
% \cline{2-3} \cline{5-6}
% Method  & Unseen (120) & Seen (480) & & Unseen (120) & Seen (480) \\
% \midrule
% Bansal~\etal~\cite{bansal2019detecting} & $11.31\pm1.03$ & $12.74\pm0.34$ && - & - \\
% % all : $12.45\pm0.16$
% \midrule
% Ours (S-S only)  & $11.85\pm1.54$ & $11.23\pm0.48$ & & $15.01\pm1.77$ & $13.66\pm0.50$ \\ 
% Ours (S-S + H app.)  & $16.72\pm1.87$ & $16.84\pm0.58$ & & $20.58\pm1.93$ & $20.36\pm0.59$ \\ 
% \bottomrule
% \end{tabular}
% % }

==> table/VCOCO_ResNet50_results.tex <==
\begin{table}[t]
\centering
\caption{\tb{Results with different feature backbone on the V-COCO $\emph{test}$ set.}
}
\label{tab:VCOCO-ResNet50}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lcccl|c}
\toprule
Method && Use human pose &&  Feature backbone & \textbf{$AP_{role}$} \\
\midrule
Ours   && - && ResNet-50         & 50.7 \\ 
Ours   && - && ResNet-50-FPN     & 51.0 \\ 
\bottomrule
\end{tabular}
% }
\end{table}

==> table/VCOCO_mAP.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Detailed results on V-COCO \emph{test} set.} The best performance is in \first{bold} and the second best is \second{underscored}.} 
% \jiarui{the score of interactiveness in github is higher than what they show in their paper. They report 48.96 in github, while in paper it is 48.7.} 
% \resizebox{0.8\columnwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
& {InteractNet~\cite{Gkioxari-CVPR-InteractNet} } & {iCAN~\cite{Gao-BMVC-iCAN}} & ${RP_{T2}C_D}^\star$~\cite{Li-CVPR-Interactiveness} & {Ours} \\
& ResNet-50-FPN & ResNet-50 & ResNet-50 & ResNet-50-FPN \\
\midrule
carry 			 & 33.1 & 32.0 & \second{40.8} &\first{41.3} \\
catch 			 & 42.5 & 47.6 & \second{48.4} &\first{49.3} \\
drink			 & 33.8 & 32.2 & \second{34.4} &\first{35.5} \\
hold 		     & 26.4 & 29.1 & \second{37.3} & \first{40.7} \\
jump  		     & 45.1 & 51.5 & \second{53.8} & \first{54.2} \\
kick  			 & \second{69.4} & 66.9 & 66.3 & \first{69.8} \\
lay   			 & 21.0 & 22.4 & \first{29.6} & \second{26.1} \\
look 			 & 20.2 & 26.5 & \second{32.3} & \first{35.5} \\
read     		 & 23.9 & \second{30.7} & 29.9 & \first{39.5} \\
ride             & 55.2 & 61.9 & \second{66.3} & \first{69.9} \\
sit              & 19.9 & 26.0 & \first{31.6} & \second{31.4} \\
skateboard       & 75.5 & 79.4 & \second{83.4} & \first{85.9} \\
ski              & 36.5 & 41.7 & \second{50.0} & \first{52.9} \\
snowboard        & 63.9 & \second{74.4} & 71.6 & \first{75.6} \\
surf             & 65.7 & 77.2 & \second{79.7} & \first{80.6} \\
talk-on-phone    & 31.8 & 52.8 & \second{53.6} & \first{55.9} \\
throw            & 40.4 & 40.6 & \second{43.3} & \first{52.1} \\
work-on-computer & 57.3 & 56.3 & \first{65.5} & \second{64.3} \\
\midrule
\multirow{2}{*}{cut} \ \ (object) & 23.0 & 34.8 & \second{40.1} & \first{42.4} \\
\qquad (instrument) & 36.4 & 37.2 & \first{41.6} & \second{39.9} \\
\multirow{2}{*}{eat} \ \ (object) & 32.4 & 37.7 & \second{39.1} & \first{41.9} \\
\qquad (instrument) & 2.0  & \second{8.3}  & \first{9.4} & 5.9  \\
\multirow{2}{*}{hit} \ \ (object) & \first{62.3} & 46.1 & 52.6 & \second{54.7} \\
\qquad (instrument) & 43.3 & 74.1 & \second{74.4} & \first{77.6} \\
\midrule
\textbf{mean AP role} & 40.0 & 45.3 & \second{49.0} & \first{51.0} \\
\bottomrule
\end{tabular}
% }
\label{tab:VCOCO}
\end{table}


==> table/VCOCO_more_ablation.tex <==
\begin{table*}[htbp]
\caption{\textbf{More Ablation study on the V-COCO \emph{val} set.} We show the $AP_{role}$. % \chen{Title looks weird.}
%\jiabin{
%(b) Show the actual number of parameters in the SSAR stream. 
%(c)
%}
}
\label{tab:more_ablation}
%
\begin{minipage}{0.5\linewidth}
{(a) \textbf{Shared SSAR modules:} Stacking more shared modules improves the performance without increasing the model size.}
\end{minipage}
%
\hfill
%
\begin{minipage}{0.45\linewidth}
{(b) \textbf{Category representation}: All of the category representation approaches achieve good performance.} 
\end{minipage}
\\
\mpage{0.45}{
\centering
\begin{tabular}{c|cc|cc}
      & \multicolumn{2}{c}{Separate} & \multicolumn{2}{c}{Shared} \\
model & S-S only & S-S + App. & S-S only & S-S + App. \\
\midrule
 1-block  & 41.1 & 46.3 & 41.1 & 46.3 \\
 \midrule
 2-block  & 43.1 & 47.4 & 43.0 & 47.3 \\
 3-block  & 43.6 & 47.5 & 43.9 & 48.1 \\
 4-block  & 43.9 & 47.9 & 44.2 & 48.1 
\end{tabular}
}
\hfill
\mpage{0.45}{ \centering
\begin{tabular}{l|cc}
 Category representation  & S-S only & S-S + App. \\
\midrule
 $\emptyset$ (no object category info.) & 13.1 & 38.8 \\
 one-hot vector                         & 39.5 & 46.0 \\
 word2vec~\cite{Mikolov-NIPS-Word2vec}  & 44.3 & 48.2 \\
 GloVe~\cite{Pennington-EMNLP-Glove}    & 44.4 & 48.1 \\
 fastText~\cite{Mikolov-LREC-fastText}  & 43.1 & 47.4 
\end{tabular}
}
\hfill
\end{table*}



==> table/obj_representation.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Object category representation.} Representing object category using word embedding works best.} 
%  \resizebox{\columnwidth}{!}{
\begin{tabular}{l|cc}
 Category representation  & S-S only & S-S + App. \\
\midrule
 $\emptyset$ (no object category info.) & 13.1 & 38.8 \\
 O app.                                 & 42.8 & 45.9 \\
 one-hot vector                         & 43.2 & 47.0 \\
 fastText~\cite{Mikolov-LREC-fastText}  & \textbf{44.3} & \textbf{47.2}
\end{tabular}
\label{tab:obj_representation}
\end{table}


==> table/word_dim.tex <==
\begin{table}[t]
\caption{\textbf{Different dimensions of the word embedding.} Performance when using different dimensions of the word embedding. We show the role mAP $AP_{role}$ on V-COCO \emph{val} set.}
\label{tab:word_dim}

\mpage{0.45}{ \centering
\begin{tabular}{l|c}
Word dim.  & S-S only \\
\midrule
10  & 45.85 \\
20  & 45.96 \\
40  & 45.99 \\
80  & 46.09 \\
160 & 46.16 \\
300 & 46.00 \\
\end{tabular}
}
\hfill
\begin{minipage}{0.45\linewidth}
{\includegraphics[width=1.0 \linewidth]{fig/dim.pdf}}
\end{minipage}
\end{table}
